PanicFI: An Infrastructure for Fixing Panic Bugs in Real-World Rust Programs

The Rust programming language has garnered significant attention due to its robust safety features and memory management capabilities. Despite its guaranteed memory safety, Rust programs suffer from runtime errors that are unmanageable, i.e., panic errors. Notably, traditional memory issues such as null pointer dereferences, which are prevalent in other languages, are less likely to be triggered in Rust due to its strict ownership rules. However, the unique nature of Rust's panic bugs, which arise from the language's stringent safety and ownership paradigms, presents a distinct challenge. Over half of the bugs in rustc, Rust's own compiler, are attributable to crash stemming from panic errors. However, addressing Rust panic bugs is challenging and requires significant effort, as existing fix patterns are not directly applicable due to the design and feature of Rust language.Therefore, developing foundational infrastructure, including datasets, fixing patterns, and automated repair tools, is both critical and urgent. This paper introduces a comprehensive infrastructure, namely PanicFI, aimed at providing supports for understanding Rust panic bugs and developing automated techniques. In PanicFI, we construct a dataset, Panic4R, comprising 102 real panic bugs and their fixes from the top 500 most-downloaded open-source crates.Then, through an analysis of the Rust compiler implementation , we identify Rust-specific patterns for fixing panic bugs, providing insights and guidance for generating patches. Moreover, we develop PanicKiller, the first automated tool for fixing Rust panic bugs, which has already contributed to the resolution of 28 panic bugs in open-source projects.The practicality and efficiency of PanicKiller confirm the effectiveness of the patterns mined within PanicFI.

==> sec/app-bak.tex <==
\subsection{Application Scenarios}
The memory-safety features of Rust offer significant benefits in systems software development. 
However, its steep learning curve and underdeveloped infrastructure pose challenges for developers and researchers in understanding the reasons behind bugs and the methods for fixing them. 
To address these issues, our work establishes a systematic infrastructure that offers a diverse dataset and comprehensive analysis of panic bugs specific to Rust projects.


Firstly, we collected a large-scale dataset of Rust panic bug fixes, \dataset, which includes fix patches from real-world projects and manually crafted code addressing a variety of root causes.
\dataset comprises $52$ reproducible panic fix cases, each containing the most concise patch and test case that can trigger panic, thereby facilitating further experiments or expansions.
The development process of \dataset mirrors that of Defects4J, a pivotal dataset in the field of APR. 
Each patch in our dataset undergoes manual verification to ensure its high quality and reliability. 
We believe that \dataset can serve as a dependable validation set for future research on automated techniques for fixing Rust panic bugs. 
Additionally, expanding \dataset to encompass other repair strategies and error types represents a promising avenue for future research.


Secondly, we have identified a series of panic bug fix patterns that align with Rust's distinctive syntax and encompass common repair strategies. 
We identified numerous potential applications for these mined patterns. For instance, they can serve as templates for pattern-based APR tools.
In this paper, we develop \tool as an application to prove the effectiveness of our mined patterns.
Additionally, these repair patterns can serve as educational resources, helping beginners to more quickly understand and fix their programs.
Moreover, the identified patterns could also contribute to a dataset for fine-tuning large language models, thus advancing AI-driven approaches in program repair and comprehension. 
This could enhance the feedback provided to developers when their programs trigger panic, improving overall developer support.


Finally, our proposed tool, \tool, is effective in real-world Rust projects, providing feedback that includes fixing patches and explanations, which are more informative than the compiler's output. 
Our experiment results for RQ3 demonstrate that \tool's efficiency in fixing panic bugs exceeds that of manual developer fixes. 
Besides, the experiments for RQ4 confirm that \tool can successfully generate fixing code for real-world, large-scale projects, with all proposed patches gaining approval from developers. 
These outcomes suggest that \tool is both practical and effective, offering significant improvements in efficiency and effectiveness for handling Rust panic bugs.

==> sec/bkg-bak.tex <==
\section{Background and Motivation}
Rust, a statically typed programming language, is gaining popularity for its well-known memory safety guarantees and high performance, making it notably distinct from C/C++ and JVM family of languages.
Memory and thread safety are ensured through a specific mechanism known as the ownership system, which naturally prevents common errors like null pointer errors.



\textbf{Motivation.}
Although there have been many APR techniques practiced on Java/C/C++, due to the unique design mechanics of the Rust language, including memory and concurrency management and type system, we consider that most of the existing repair patterns are not applicable on Rust programs.
Specifically, the \texttt{null} in Java is used to indicate the state of a variable that does not point to any object. 
All reference variables can be set to \texttt{null}, which means that they do not refer to any object in memory. 
While this design is convenient for representing uninitialized state in some cases, it also poses a number of problems, and most of Java's fix patterns revolve around checking for null values to avoid the null pointer exception~\cite{liu2019tbar, koyuncu2019ifixr, kim2013par, liu2019avatar}.
\liu{Add more ref.}
For example, the function in Listing~\ref{lst:motiv_java} tries to return a null value while the expected return type is \texttt{int}.
This would trigger a very common null pointer bug, and the existing APR technique generally adds an extra condition to check if the \texttt{value} is a \texttt{null}, then return random data which fits the return type requirement.

\begin{listing}[h]
\begin{minted}[linenos=false,
%frame=single,
fontsize=\small,
highlightcolor=green!10,
highlightlines={4,5,6}]{java}
public class Buggy {
    public static int test() {
        Integer value = null;  // Not allowed in Rust
+       if (value == null) {  // Exisiting fix pattern
+           return 0;
+       } 
        return value; // NullPointerException
    }
}
\end{minted}
\caption{A minimized Java program triggering null pointer exception and the corresponding fix patch.} \label{lst:motiv_java}
%\vspace{-5mm}
\end{listing}

However, due to differences in language design mechanisms, Rust programs are much stricter in the definition and use of \texttt{null} values.
Rust has no direct notion of \texttt{null}; instead, the data type \texttt{Option<T>} is used to explicitly handle cases where values may not exist.
As shown in the following code snippet, if the data is potentially null, it has to be wrapped in the \texttt{Option<T>} and using the \texttt{match} pattern to safely process its value.
The language design naturally avoids the null pointer bug in safe Rust, thus, existing fix patterns are completely ineffective on Rust programs. 

\begin{listing}[h]
\begin{minted}[linenos=false,
%frame=single,
fontsize=\small]{rust}
fn test() -> i32 {
    let value: Option<i32> = Some(1);  // Potentially null
    match value {
        Some(v) => v, // if it's some value, then return it
        None => 0,    // if it's None, then return 0
    }
}
\end{minted}
\caption{An example of handling null values in Rust, naturally preventing the most frequent null pointer bugs in Java.} \label{lst:motiv_rust}
%\vspace{-5mm}
\end{listing}

Besides, we notice that the C/C++ bug fixing task's dataset, CVEFixes~\cite{}, covers a wide variety of memory bugs such as improper restriction of operations within the bounds of a memory buffer (CWE-119), out-of-bounds write (CWE-787), and NULL pointer dereference (CWE-476), etc., but these bugs wouldn't be triggered in safe Rust programs, leading to the existing fix patterns invalid.


==> sec/exp-bak.tex <==
\subsection{Experiment Design}
In this section, we illustrate our research questions and the baseline approaches employed in our experiments.
We have implemented \tool with Rust, and captured Rust's High-level Intermediate Representation (HIR)~\cite{hir:online}, which is a special representation used in the Rust compiler, to construct the dependency graph of suspicious locations.
In addition, we implement the visiting and modification of the AST nodes based on the AST manipulation library syn~\cite{syn:online}, to generate the fix patches.
All the experiments are constructed on a Ubuntu 20.04.1 LTS laptop with 11th Gen Intel(R) Core(TM) i5-11300H @3.10GHz CPU.



\subsection{Research Questions}
\tool is designed to automatically fix Rust panic bugs. 
To this end, we empirically explore the following research questions (RQ):

\textit{\textbf{RQ1 (Fault Localization)}: To what extent does \tool provide reliable fault localization results for panic bugs fixing?}
In this RQ, we aim to evaluate the accuracy of our bug localization approach based on stacktrace information and dependency analysis.
We categorize the real data in \dataset into small-scale datasets ($ < 20$K LoC) and large-scale datasets ($\geq 20$K LoC) based on the size of the source code.
% \liu{@yb: check the LoC here}
We present the accuracy of various localization approaches at top-1, top-3, and top-5 levels.
The accuracy is calculated based on three granularity levels: files, statements, and expressions.
% We present the accuracy of various localization approaches, categorizing them into top1, top3, and top5, respectively. 
% The accuracy is calculated based on the granularity of the localization, specifically considering the localization level of files, statements, and expressions.


\textit{\textbf{RQ2 (Fixing Effectiveness)}: How effective is \tool for fixing panic bugs compared to state-of-the-art LLM-based techniques?}
To evaluate \tool's effectiveness, we first verified the accuracy of patches it generated on \dataset. Additionally, we conducted comparative experiments to assess patch generation accuracy when correct error localization information was given to both \tool and baseline methods.
Referring to existing research on APR~\cite{qi2015plausible}, we categorize the fixes into three types and verify their proportion: (1) panic-eliminated patches, where the panic bug is resolved but some regression test cases fail; (2) plausible patches, where the panic bug is successfully fixed and all test cases pass; and (3) correct patches, which are plausible patches that have also been manually verified for semantic correctness.
% Besides, we also report the number of generated patches which are exactly same as the collected patch in \dataset.



\textit{\textbf{RQ3 (Efficiency)}: What is the fixing efficiency of \tool compared with traditional manual repair methods?} 
% To address the difficulty of locating and understanding the fixes for panic bugs, we apply \tool to assist in automating the fixes for panic bugs.
In this RQ, we measure the time required to apply \tool for fixing each target, and compare it with the duration from when the issue was reported to the PR was merged.
This comparison aims to assess the extent to which our proposed approach enhances the efficiency of bug repairing.



\textit{\textbf{RQ4 (Case Study)}: Can \tool be applied to the real-world Rust projects and fix practical panic bugs?}
% \liu{We need to update this paragraph}
% As the first automated fixing tool particularly designed for Rust panic bugs, 
To evaluate the practical effectiveness, we apply \tool to fix real-world issues in GitHub, which are not included in \dataset. 
For open issues, we submit a PR with the fix patch generated by \tool, and we track whether they are confirmed and merged by developers. 
For closed issues, we use TF-IDF~\cite{sparck1972statistical} to calculate the similarity between the generated patch with the official patch. 
If the score exceeds $0.75$, and the panic is fixed with the regression test passed, we consider they are similar. 
If the PR is accepted by project developers or if our generated patch is similar to the official patch, it could further demonstrate that \tool can be employed to real-world application scenarios and provide fixing guidance for large-scale real-world projects.

\subsection{Baseline Approaches}
For the task of bug localization, while existing techniques typically rely on additional natural language descriptions from bug reports or test suites~\cite{yoo2012regression}, our tool, \tool, solely utilizes the error message from the Rust compiler and the accompanying stacktrace information. 
% Furthermore, existing techniques are designed for languages like C, C++, Java, and Python, they are not tailored to handle panic errors in Rust, which have distinct error message characteristics.
The absence of extra data makes some existing techniques unsuitable as baselines for our approach. 
Consequently, we select three categories of general methods as baseline techniques to compare with the fault localization capabilities of \tool.
% Consequently, we devised three baseline methods based on conventional localization approaches:
% (1) \textit{panic}: Directly using the location indicated in the panic error message.
% (2) \textit{random}: Randomly selecting a suspicious location from the stacktrace.
% (3) \textit{similarity}: Calculating textual similarity between the error message and each code location; the highest similarity score indicates the fault location.

\textbf{(1) Conventional Localization Approaches.} When only error messages and stacktraces are available, fault localization can be deduced from these elements. We outline three fundamental techniques below: \liu{add cites}
\begin{itemize}
\item \textit{Panic}: When a panic occurs in a Rust program, the compiler outputs an error message indicating the specific line of code where the exception occurred. This identified line is then considered the fault location.
\item \textit{Random}: Upon a panic in a Rust program, the compiler outputs stacktrace information that includes a list of suspicious code locations. From this list, a location is randomly selected as the detected fault location.
\item \textit{Similarity}: We assess the textual error message to compute the similarity between the message and each code location. The location with the highest similarity score is determined to be the fault location.
\end{itemize}


\textbf{(2) Spectrum-based Localization Approaches.} 
Spectrum-based fault localization (SBFL)~\cite{abreu2007spectrum} approaches analyze the execution traces of a program by examining which components of the program were executed when a failure occurred and which were not. The spectrum refers to the range of execution traces collected during test runs. By applying statistical analysis to these execution spectra, SBFL effectively pinpoints the components that are most likely to be responsible for software failures. 
In our experiments, we collect test cases for each crate in \dataset, the majority of which passed; those that triggered a panic bug were classified as failed cases.
Based on the calculated scores from the spectral analysis, we sort all the lines of code and then select the top 5 locations as the fault localization results.
Due to slight variations in how the spectrum is calculated, we select the two most commonly used metrics as our baselines.
\begin{itemize}
\item \textit{Tarantula}: The Tarantula method~\cite{jones2002tarantula} calculates the suspicious location by comparing the ratios of passed to failed test cases that execute a given code line. A higher ratio of failed to total test executions in a component increases its likelihood of being faulty. We rank the ratio of each code line as the most likely fault candidates.
\item \textit{Ochiai}: The Ochiai algorithm~\cite{meyer2004comparison} applies the cosine similarity measure between failed test cases and the execution of given code lines. The score is derived from the intersection of failing test cases with the components they execute, normalized by the square root of the product of the total number of failures and the number of times a component is executed during those failures. 
\end{itemize}

\textbf{(3) LLM-based Localization Approaches.} With the rapid advancement of Large Language Models (LLMs), it is feasible to directly submit source code, error messages, and requirements to an LLM. In response, the LLM could generate corresponding fault localization results.
\begin{itemize}
\item \textit{ChatGPT-4 (GPT-4)}: Due to ChatGPT-3.5's limitations in handling files, we apply the most popular commercial software ChatGPT 4.0 as a baseline.
\item \textit{Multiple rounds of inquiries with ChatGPT-4 (GPT4-multi)}: When interacting with ChatGPT 4.0, we inquire multiple rounds with additional questions manually.
\end{itemize}


% To the best of our knowledge, no existing tools specifically address bug localization or the automated repair of Rust panic bugs. 
% We therefore benchmark against the state-of-the-art LLM-based technique, ChatGPT. 
% Due to ChatGPT-3.5's limitations in handling files, we utilize the advanced and commercial ChatGPT-4.0 as our primary baseline. 
As for the automatic repairing task, existing patterns for other programming languages are not applicable for Rust panic bugs, thus, we mainly compare the effectiveness of \tool with LLM-based approaches.
We follow a standardized process when applying ChatGPT 4.0 as a baseline method for fault localization and program repair.
For each target, we upload a zip archive containing the entire Rust project, the test case triggering the panic, and relevant panic information. 
We then use a consistent prompt template, as shown below:

% To the best of our knowledge, there are no existing tools for bug localization or automated fixing of Rust panic bugs, so we compare the effectiveness of bug localization and fixing with the state-of-the-art LLM-based technique, i.e., ChatGPT.
% Because ChatGPT-3.5 does not support receiving files, we apply the latest version of the commercial ChatGPT-4.0 as a major baseline.
% For each target, we upload a zip archive of the entire Rust project, the test case that triggers panic, and the panic information.
% Then, we employ a consistent prompt template, as illustrated below:




\begin{framed}
\footnotesize \textsf{I have uploaded a source code package of a Rust crate \textbf{[crate-name]}, \textbf{[crate-zip]}. When using this crate with the following test case: \textbf{[main.rs]}, it went panic, the panic information is as follows: \textbf{[panic\_info]}.}

\footnotesize \textsf{\textbf{[Location Prompt]} + Based on the locations, provide the top 5 \textbf{fixing code} to fix this panic. Don't explain anything about code, just show me the suspicious locations and patches.}
\end{framed}

As for the \textbf{[Location Prompt]}, because we verify the correctness of the generated patches with/without the correct error location, the template are specifically as follows:

\begin{framed}

\begin{itemize}[leftmargin=*]
    \item \footnotesize \textbf{Without Perfect Location}: \textsf{Please give me the top 5 \textbf{suspicious fault locations} in the crate, including their path, line number and column number.} 
    \item \footnotesize \textbf{With Perfect Location}: \textsf{The error location is: \textbf{[perfect-location]}.}
\end{itemize}

\end{framed}


Because ChatGPT may fail to produce bug localization or repair patches as instructed, we employ a baseline involving multiple interactions with ChatGPT. 
Initially, we assess ChatGPT's output for completeness and iterate the query process up to three times, correcting for any missing information. 
If, after three attempts, localization or repair details remain unattained, we classify the effort as a ChatGPT repair failure. 
The inquiry prompts for missing information are as follows:


% According to our experiments, ChatGPT may fail to produce bug localization or repair patches as instructed. 
% For this reason, we also employ another baseline involving multiple rounds of interactions with ChatGPT. 
% After the initial round, we manually review ChatGPT's output for any missing information, then query ChatGPT again until all necessary information is obtained, but no more than three times in total. 
% If no localization or repair information is acquired after three queries, we regard it as a ChatGPT repair failure. The inquiry prompts for missing information are as follows:



\begin{framed}

\begin{itemize}[leftmargin=*]
\item \footnotesize \textsf{\textbf{Localization}: Please provide me directly with the exact \textbf{file path}, \textbf{code line} and \textbf{column numbers} where the error was located.}

\item \footnotesize \textsf{\textbf{Fixing}: Based on the mislocalization information you provided, please provide me with the specific code to fix it.}
\end{itemize}

\end{framed}

\section{Result Analysis}
\input{sec/result} 


==> sec/result-bak.tex <==
In this section, we present the experiment results on automatically fixing panic bugs and then analyze the effectiveness and efficiency our proposed tool \tool.

\begin{table*}[htbp]
\centering
\caption{The correct number and correctness of different tools on real and synthetic datasets, respectively, with different granularities of error localization.}
\label{tab:rq1}
\footnotesize
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{cc|ccc|ccc|ccc||ccc}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Tool}}} & \multicolumn{3}{c|}{\textbf{Real Dataset-Small (30)}}     & \multicolumn{3}{c|}{\textbf{Real Dataset-Large (22)}}    & \multicolumn{3}{c||}{\textbf{Synthetic Dataset (40)}}    & \multicolumn{3}{c}{\textbf{Total (92)}}    \\ \cline{3-14} 
&& File  & Stmt  & Expr  & File  & Stmt  & Expr  & File   & Stmt  & Expr  & File  & Stmt & Expr  \\ \hline
\multirow{6}{*} {Top-1} & panic        & 24 (80.0\%) & 17 (56.7\%) & 17 (56.7\%) & 14 (63.6\%) & 10 (45.5\%) & 10 (45.5\%) & 39 (97.5\%) & 38 (95.0\%) & 36 (90.0\%) & 78 (84.8\%) & 65 (70.7\%) & 63 (68.5\%) \\ 
&random       & 14 (46.7\%) & 4 (13.3\%)  & 3 (10.0\%)  & 11 (50.0\%) & 5 (22.7\%)  & 4 (18.2\%)  & 39 (97.5\%)  & 35 (87.5\%) & 35 (87.5\%) & 64 (69.6\%) & 44 (47.8\%) & 42 (45.7\%) \\ 
&NLP          & 4 (13.3\%)  & 0 (0\%)     & 0 (0\%)     & 4 (18.2\%)  & 1 (4.5\%)   & 0 (0\%)     & 39 (97.5\%)  & 5 (12.5\%)  & 2 (5.0\%)   & 47 (51.1\%) & 6 (6.5\%)   & 2 (2.2\%)   \\ 
&GPT-4        & 22 (73.3\%) & 18 (60.0\%) & 13 (43.3\%) & 7 (31.8\%)  & 4 (18.2\%)  & 3 (13.6\%)  & \textbf{40 (100.0\%)} & 35 (87.5\%) & 34 (85.0\%) & 69 (75.0\%) & 57 (62.0\%) & 44 (47.8\%) \\ 
&GPT4-multi   & 22 (73.3\%) & 18 (60.0\%) & 13 (43.3\%) & 7 (31.8\%)  & 4 (18.2\%)  & 3 (13.6\%)  & \textbf{40 (100.0\%)} & 35 (87.5\%) & 34 (85.0\%) & 69 (75.0\%) & 57 (62.0\%) & 50 (54.3\%) \\ 
&\textbf{\tool}  & \textbf{25 (83.3\%)} & \textbf{21 (70.0\%)} & \textbf{20 (66.7\%)} & \textbf{15 (68.2\%)} & \textbf{11 (50.0\%)} & \textbf{11 (50.0\%)} & 39 (97.5\%)  & \textbf{39 (97.5\%)} & \textbf{39 (97.5\%)} & \textbf{79 (85.9\%)} & \textbf{71 (77.2\%)} & \textbf{70 (76.1\%)} \\ \midrule
\multirow{5}{*} {Top-3} & random       & 24 (80.0\%) & 15 (50.0\%) & 15 (50.0\%) & 12 (54.5\%) & 6 (27.3\%)  & 6 (27.3\%)  & 39 (97.5\%)  & 37 (92.5\%) & 37 (92.5\%) & 75 (81.5\%) & 58 (63.0\%) & 58 (63.0\%) \\ 
& NLP          & 8 (26.7\%)  & 0 (0\%)     & 0 (0\%)     & 7 (31.8\%)  & 1 (4.5\%)   & 0 (0\%)     & 39 (97.5\%)  & 13 (32.5\%) & 3 (7.5\%)   & 54 (58.7\%) & 14 (15.2\%) & 3 (3.3\%)   \\ 
&GPT-4        & 22 (73.3\%) & 19 (63.3\%) & 14 (46.7\%) & 8 (36.4\%)  & 4 (18.2\%)  & 3 (13.6\%)  & \textbf{40 (100.0\%)} & 38 (95.0\%) & 37 (92.5\%) & 70 (76.1\%) & 61 (66.3\%) & 54 (58.7\%) \\ 
&GPT4-multi   & 22 (73.3\%) & 19 (63.3\%) & 14 (46.7\%) & 8 (36.4\%)  & 4 (18.2\%)  & 3 (13.6\%)  & \textbf{40 (100.0\%)} & 38 (95.0\%) & 37 (92.5\%) & 70 (76.1\%) & 61 (66.3\%) & 54 (58.7\%) \\ 
&\textbf{\tool}  & \textbf{26 (86.7\%)} & \textbf{22 (73.3\%)} & \textbf{21 (70.0\%)} & \textbf{17 (77.3\%)} & \textbf{13 (59.1\%)} & \textbf{13 (59.1\%)} & 39 (97.5\%)  & \textbf{39 (97.5\%)} & \textbf{39 (97.5\%)} & \textbf{82 (89.1\%)} & \textbf{74 (80.4\%)} & \textbf{73 (79.3\%)} \\ \midrule
\multirow{5}{*} {Top-5} & random       & \textbf{26 (86.7\%)} & 19 (63.3\%) & 19 (63.3\%) & 14 (63.6\%) & 10 (45.5\%) & 9 (40.9\%)  & 39 (97.5\%)  & 37 (92.5\%) & 37 (92.5\%) & 79 (85.9\%) & 66 (71.7\%) & 65 (70.7\%) \\ 
&NLP          & 9 (30.0\%)  & 0 (0\%)     & 0 (0\%)     & 10 (45.5\%) & 1 (4.5\%)   & 0(0\%)      & \textbf{40 (100.0\%)} & 23 (57.5\%) & 6 (15.0\%)  & 59 (64.1\%) & 24 (26.1\%) & 6 (6.5\%)   \\
&GPT-4        & 24 (80.0\%) & 20 (66.7\%) & 14 (46.7\%) & 10 (45.5\%) & 4 (18.2\%)  & 3 (13.6\%)  & \textbf{40 (100.0\%)} & \textbf{39 (97.5\%)} & 38 (95.0\%) & 74 (80.4\%) & 63 (68.5\%) & 55 (59.8\%) \\
&GPT4-multi   & 24 (80.0\%) & 20 (66.7\%) & 14 (46.7\%) & 10 (45.5\%) & 4 (18.2\%)  & 3 (13.6\%)  & \textbf{40 (100.0\%)} & \textbf{39 (97.5\%)} & 38 (95.0\%) & 74 (80.4\%) & 63 (68.5\%) & 55 (59.8\%) \\ 
&\textbf{\tool}  & \textbf{26 (86.7\%)} & \textbf{22 (73.3\%)} & \textbf{21 (70.0\%)} & \textbf{17 (77.3\%)} & \textbf{13 (59.1\%)} & \textbf{13 (59.1\%)} & 39 (97.5\%)  & \textbf{39 (97.5\%)} & \textbf{39 (97.5\%)} & \textbf{82 (89.1\%)} & \textbf{74 (80.4\%)} & \textbf{73 (79.3\%)} \\ \bottomrule
\end{tabular}}
\end{table*}

\subsection{Answer to RQ1: Fault Localization} \label{subsec:rq1}
To comprehensively assess the impact of fault localization through various techniques, we designated three distinct levels of granularity for locating panics: file, statement, and expression levels. 
% Additionally, we factored in the precision of recommendations, thereby categorizing them into top1, top3, and top5 rankings, respectively.
% Table~\ref{tab:rq1} presents the experiment results.

% The granularity of fault localization, represented by different levels, plays a crucial role in the effectiveness and efficiency of Automated Program Repair (APR) tools. 
% As highlighted by Koyuncu et al.~\cite{koyuncu2019ifixr}, the granularity at which faults are localized can significantly influence the adoption and success of APR in both research and practical applications. 
% The iFixR algorithm, for instance, focuses on statement-level fault localization. However, our experimental findings suggest that statement-level localization may not be sufficiently precise for optimal APR performance. This is particularly evident when examining the differences between statement and expression-level results. A single statement, such as a complex if expression, can be lengthy and encompass multiple potential fault sites, where the actual error may only pertain to a small segment of it. 

As illustrated in Table~\ref{tab:rq1}, \tool demonstrates consistent accuracy at both the statement and expression levels, surpassing other methods like GPT-4 and NLP, which indicates the hidden limitations of these tools. Localization at the file level is deemed too broad for effective fault isolation, given that a single source code file can contain thousands of lines. 



Among the top-5 recommendations by NLP techniques, correct patches at the file level significantly lag behind those identified at the statement and expression levels, with correct expression-level fixes constituting only 10\% (6 out of 59) of those correctly located at the file level. 

The difference observed between the first two real datasets and the manually synthesized dataset sheds light on the practical efficacy of APR tools in addressing complex issues, a crucial determinant of their applicability in real-world scenarios. Notably, the performance of the random technique varies significantly across these datasets. While it achieves commendable accuracy on the synthetic dataset—surprisingly surpassing \tool at the file level—its effectiveness markedly diminishes when applied to real datasets. Here, \tool consistently outperforms the random technique across all levels of fault localization and recommendation tiers. This discrepancy highlights the inherent challenges of fault localization in authentic repair situations. Specifically, the depth of the stack backtrace and the overall size of the Rust program emerge as pivotal factors that influence the success of fault localization strategies. In real-world fixing scenarios, for instance, the average size of the programs in our dataset, \dataset, spans approximately 29,073 lines of code. This considerable size not only extends the stack backtrace but also expands the code search space, thereby increasing the complexity of fault localization compared to scenarios involving manually crafted synthetic datasets. Consequently, the observed differences underscore the necessity for APR tools to adeptly navigate the intricate landscapes of real-world codebases, where the challenges of scale and complexity profoundly impact their performance and utility.

One of the emerging trends in APR research is the adoption of learning-based approaches, among which techniques powered by Large Language Models (LLMs) have demonstrated significant promise. In our study, we utilized GPT-4 developed by OpenAI by providing it with the complete source code and detailed panic error messages. Intuitively, one might anticipate that such comprehensive inputs would enable GPT-4 to outperform the panic method within real dataset contexts. However, contrary to expectations, GPT-4's performance was notably inferior to approaches that simply utilized locations in error messages. Throughout our experiments with GPT-4, we even encountered challenges in its failure in analyzing crate source code, suggesting a potential shortfall in its ability to dissect and comprehend large-scale Rust programs effectively. To mitigate any variability stemming from the inherent randomness of LLMs, we extended our experiment to include multiple iterations with GPT-4. The consistency of the results across these rounds further corroborated the observation that GPT-4 struggles with interpreting complex project structures. Interestingly, when provided with smaller code snippets from a synthetic dataset, GPT-4's performance saw a marked improvement. In the context of the synthetic dataset, GPT-4 exhibites superior performance at the file level compared to \tool. Since most of the cases in synthetic database contains only a few files, this outcome suggests that the effectiveness of GPT-4 in this scenario may be influenced not solely by the size of the source code but also by the necessity to analyze across multiple files.  This dichotomy underscores a critical insight: while LLM-based techniques like GPT-4 hold substantial potential for APR, their current effectiveness appears constrained by the scale and complexity of the projects in question. These findings highlight a crucial area for future enhancement, suggesting that refining LLMs' comprehension abilities for large-scale codebases could significantly amplify their utility in real-world software development and maintenance scenarios.




\subsection{Answer to RQ2: Fixing Effectiveness}
In Table~\ref{tab:rq2}, we evaluate each method across three dimensions using a real dataset. Due to the absence of regression tests for the synthetic dataset, it's challenging to definitively assess the correctness of the patches generated.

Overall, it becomes clear that \tool significantly surpasses the performance of automated repairs conducted by GPT-4, including its iterative applications, across all evaluated datasets. Particularly noteworthy is the observation within large real datasets, where GPT-4 fails to produce even a single viable patch. This deficiency is closely tied to GPT-4's challenges with fault localization, as elaborated in Section~\ref{subsec:rq1}. Moreover, it's crucial to emphasize the nature of GPT-4's repair strategies when addressing large-scale Rust programs. Typically, GPT-4's approach involves altering the program logic without a comprehensive consideration of the entire project's context. For instance, it might change a method's return type, leading to compilation errors that can compromise the project's integrity, or it might introduce new logic that overlooks the program's designed encapsulation principles. These rough fixes lead to the compilation failure of the whole Rust project, not to mention whether the patch is plausible or not. The outcomes derived from the synthetic dataset further demonstrates this point. GPT-4 is capable of generating several plausible patches, albeit not identical to the expected solutions, showcasing its proficiency in addressing panic scenarios. Nevertheless, it's crucial to note that the scale of the synthetic dataset is substantially smaller compared to the real datasets. Moreover, the complexity of cases within the synthetic dataset tends to be relatively low, usually revolving around a singular logic or functionality. This simplification eliminates many of the intricacies and challenges present in real-world applications, consequently painting a more favorable picture for GPT-4's performance. This distinction highlights the essential consideration that GPT-4’s capabilities to fix panics, while promising under controlled or simplified conditions, may not directly translate to the same level of success in the more complex and multifaceted environments typical of real-world software development. Like Sec~\ref{subsec:rq1}, we conducted iterative applications of GPT-4 and sadly no substantial improvement has emerged.

The emergence of patches that aren't plausible can be partly attributed to the oversight of fix patterns, which inherently reflects the limitations of pattern-based APR methods: their effectiveness is confined to the scope of identified patterns. However, it also highlights a broader challenge in APR—achieving a balance between the specificity of fix patterns, which ensures the relevance and applicability of patches, and the need for a comprehensive catalog that can address the diverse and dynamic nature of software bugs. Moreover, the complexity of APR challenges is further illustrated by patches that necessitate modifications across multiple locations, potentially triggering a domino effect within the codebase. For instance, one of the unsuccessful patches we generated involved adding an as\_bytes() method call to a variable as its return value—a modification identical to what a developer had implemented. However, the subsequent "chain reaction," necessitating adjustments to the return type, fell outside our automated tool's capability, underlining a task requiring manual intervention. This scenario underscores a significant hurdle in APR, namely addressing non-source bug fixes, a category of issues that extend beyond the direct source code modifications typically targeted by APR tools, as identified in the literature~\cite{yoo2012regression, huang2023survey}. These non-source modifications represent a frontier that current APR technologies have yet to conquer. 

One of the critical challenges currently confronting the field of APR research is the quality of the patches produced by the developed tools, a factor that significantly impacts their practical applicability in real-world repair scenarios. Prior studies, such as the work by Yoo et al.~\cite{yoo2012regression}, have advocated for the use of regression testing as a means to ensure that modifications do not adversely affect the existing behavior of the original program. Following this approach, we employ regression testing as a benchmark to evaluate the correctness of generated patches. \tool outperforms GPT-4 in terms of producing correct patches, a result that is particularly encouraging given that over half of the patches deemed plausible by our tool were also verified to be correct. However, it is noteworthy that GPT-4 demonstrates a higher proficiency in ensuring that its plausible patches are not only potentially viable but are indeed correct. This distinction could be attributed to the inherent limitations within \tool's pattern-based approach. For instance, adjusting the return error type in the wildcard arm of a match expression might not correspond accurately to the program's design goals, leading to failures in certain test cases that focus on error handling. 

Additionally, we conduct manual reviews of patches derived from pull requests to verify the congruence of our solutions with those authored by developers. It is imperative to acknowledge that discrepancies between our automated fixes and those found in pull requests do not inherently denote inaccuracies on our part. There exists a possibility that a patch, while not identical to the developer-provided solution, can still be correct and functionally viable. This scenario underscores the multifaceted nature of software repair, where multiple pathways can lead to a valid solution, reflecting the diversity and creativity inherent in programming. 

\begin{table*}[htbp]
\centering
\caption{The number of correct patches and correctness of different tools on real and synthetic datasets, respectively.} 
\label{tab:rq2}
\setlength{\tabcolsep}{0.9mm}{ 
\begin{tabular}{cc|ccc|ccc|cc||cc}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Tool}}} & \multicolumn{3}{c|}{\textbf{Real Dataset-Small (30)})}                                         & \multicolumn{3}{c|}{\textbf{Real Dataset-Large (22)}}                                       & \multicolumn{2}{c||}{\textbf{Synthetic Dataset (40)}}             & \multicolumn{2}{c}{\textbf{Total (92)}}                \\ \cline{3-12} 
                  && Same       & Correct     & Plausible   & Same       & Correct    & Plausible &Same & Plausible     &Same & Plausible   \\ \hline
\multirow{3}{*} {Top-1}
& GPT-4        & 0 (0\%)    & 6 (20.0\%)  & 6 (20.0\%)  & 0 (0\%)    & 0 (0\%)    & 0 (0\%)    & 8 (20.0\%)  & 29 (72.5\%) & 8 (8.7\%)   & 35 (38.0\%) \\
& GPT-4 (multi)   & 0 (0\%)    & 7 (23.3\%)  & 7 (23.3\%)  & 0 (0\%)    & 0 (0\%)    & 0 (0\%)    & 8 (20.0\%)  & 29 (72.5\%) & 8 (8.7\%)   & 36 (39.1\%) \\
& \textbf{\tool}  & 0 (0\%)    & \textbf{9 (30.0\%)}  & \textbf{18 (60.0\%)} & \textbf{2 (9.1\%)}  & \textbf{3 (13.6\%)} & \textbf{5 (22.7\%)} & \textbf{28 (70.0\%)} & \textbf{30 (75.0\%)} & \textbf{30 (32.6\%)} & \textbf{53 (57.6\%)} \\ \midrule
\multirow{3}{*}{Top-3}
& GPT-4        & 1 (3.3\%)  & 6 (20.0\%)  & 6 (20.0\%)  & 0 (0\%)    &0 (0\%)    & 0 (0\%)    & 10 (25.0\%) & 32 (80.0\%) & 11 (12.0\%) & 38 (41.3\%) \\
& GPT-4 (multi)   & 1 (3.3\%)  & 7 (23.3\%)  & 7 (23.3\%)  & 0 (0\%)   & 0 (0\%)    & 0 (0\%)    & 10 (25.0\%) & 32 (80.0\%) & 11 (12.0\%) & 39 (42.4\%) \\
& \textbf{\tool} & \textbf{5 (16.7\%)} & \textbf{13 (43.3\%)} & \textbf{21 (70.0\%)} & \textbf{5 (22.7\%)} & \textbf{5 (22.7\%)} & \textbf{8 (36.4\%)} & \textbf{36 (90.0\%)} & \textbf{36 (90.0\%)} & \textbf{46 (50.0\%)} & \textbf{65 (70.7\%)} \\ \midrule
\multirow{3}{*}{Top-5}
& GPT-4        & 1 (3.3\%)  & 6 (20.0\%)  & 6 (20.0\%)  & 0 (0\%)    & 0 (0\%)    & 0 (0\%)    & 11 (27.5\%) & 32 (80.0\%) & 12 (13.0\%) & 38 (41.3\%) \\
& GPT-4 (multi)  & 1 (3.3\%)  & 7 (23.3\%)  & 7 (23.3\%)  & 0 (0\%)    & 0 (0\%)    & 0 (0\%)    & 11 (27.5\%) & 32 (80.0\%) & 12 (13.0\%) & 39 (42.4\%) \\
& \textbf{\tool}  & \textbf{5 (16.7\%)} & \textbf{14 (46.7\%)} & \textbf{22 (73.3\%)} & \textbf{5 (22.7\%)} & \textbf{5 (22.7\%)} & \textbf{9 (40.9\%)} & \textbf{36 (90.0\%)} & \textbf{36 (90.0\%)} & \textbf{46 (50.0\%)} & \textbf{77 (83.7\%)} \\ \bottomrule
\end{tabular}}
\end{table*}


\subsection{Answer to RQ3: Efficiency}
Fig~\ref{fig:rq3} and Table~\ref{tab:rq3} illustrate the time efficiency of \tool compared to the duration required for manual fixes. It's noteworthy to mention that no actual fix data is available for the synthetic dataset. The data presented in Table~\ref{tab:rq3} highlight \tool's capability to significantly reduce the repair time from an average of several days to mere minutes. Specifically, Fig~\ref{fig:rq3} vividly depicts the distribution of fix times, emphasizing the median repair time. This median value reveals that \tool necessitates less than a minute to address fixes, starkly contrasting with manual repair efforts that can span several days.

The observation that the fix times for smaller real datasets appear longer than those for larger ones may initially seem counter-intuitive. However, this phenomenon is clarified upon closer examination of Fig~\ref{fig:rq3}, which indicates a higher incidence of outliers in the smaller dataset compared to the larger one. In fact, certain crates within the smaller dataset necessitate protracted fix duration when addressed by \tool, attributable to their intricate test suites requiring thorough validation processes. This scenario sheds light on the methodology behind constructing \dataset, wherein only closed issues were considered. Consequently, the larger dataset might ignore those open or repeatedly reopened issues, contributing to its seemingly quicker fix times. Both Fig~\ref{fig:rq3} and Table~\ref{tab:rq3} corroborate the result that synthetic dataset cases are resolved more swiftly. The synthetic dataset, characterized by its smaller codebase size, leads to a reduced stack backtrace length and simpler logical structures. This simplicity effectively circumvents the complexities associated with cross-file dependencies, a common challenge in real-world programming scenarios.

In examining the intricacies of real-world pull request workflows, we have identified several interesting factors that significantly influence the duration required to finalize a fix. Among these, the interaction and discussions between developers stand out as a critical element. Often, developers may find it challenging to comprehend the code written by their peers without comprehensive explanations, a situation that stems from issues related to patch interpretability. This challenge is currently a significant hurdle within the APR domain~\cite{huang2023survey}. In response, \tool aims to mitigate this challenge by providing detailed explanations alongside the fix patches, thereby facilitating a smoother review process and enhancing understanding among developers. Another noteworthy observation pertains to instances where maintainers request multiple revisions of a submitted fix, sometimes suggesting entirely different approaches. This aspect of the review process can significantly extend the time taken to achieve a consensus on the appropriate fix. Here, the recommendation list generated by \tool emerges as a valuable resource. By offering a variety of potential fixes, \tool can potentially streamline the decision-making process, enabling developers and maintainers to quickly identify and agree upon the most suitable solution, thereby reducing the time and iterations needed for approval. These meaningful insights will be applied in Section~\ref{subsec:ans_rq4}, where we applied \tool into a real-world workflow and details between developers and us will be presented there.

\begin{table}[htbp]
\centering
\small
\caption{Time consuming for \tool and actual bug fixes.} \label{tab:rq3}
\begin{tabular}{ccccc}
\toprule
\textbf{Datasets}    & \textbf{Approaches}   & \textbf{Min} & \textbf{Max}     & \textbf{Avg.}  \\ \midrule
\multirow{2}{*}{\textbf{Real Dataset-Small}} & \tool & 1.77s   & 588.72s     & 142.00s     \\
 & Actual     & 0.73h    & 807 days & 76 days \\ \hline
\multirow{2}{*}{\textbf{Real Dataset-large}} & \tool & 3.34s  & 178.22s     & 51.5s      \\
& Actual      & 0.88h   & 61 days   & 10 days \\ \hline
\textbf{Synthetic Dataset}      & \tool & 0.72s        & 2.36s        & 1.33s     \\ \bottomrule
\end{tabular}
\end{table}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/rq3_boxplot.pdf}
    \caption{Experiment results of efficiency.}
    \label{fig:rq3}
\end{figure}

\subsection{Answer to RQ4: Case Study} \label{subsec:ans_rq4}
To prove \tool's practical effect on large-scale Rust program, we applied it to open issues within open-source Rust projects. Up to this point, \tool has achieved notable success, having rectified four panic bugs. These fixes have not only been approved by the project maintainers but have also been incorporated into subsequent version releases. The four panic bugs that \tool successfully addressed span a variety of common root causes, including arithmetic overflow, index out of bounds, and unwrapping on None or other invalid values.

The subsequent two patches were contributed to a Rust crate hifitime~\ref{}, which boasts over 11,000 lines of code and has accumulated a total of 173,613 downloads. 

Listing~\ref{lst:rq4-1} showcases the resolution of an array out-of-bounds error, with a code snippet and error message as follows:

\textsf{
thread 'main' panicked at 'begin <= end (21 <= 20) when slicing `94-11-05T08:15:34.0-:0`', /path/hifitime-3.8.2/src/epoch.rs:993:43
}

To begin addressing this issue, we executed the code snippet with the environment variable RUST\_BACKTRACE=full set, enabling us to capture a detailed backtrace along with the panic error message. Armed with this crucial information, we initiated \tool. The first step undertaken by \tool involved constructing a dependency graph for hifitime, which was subsequently stored in a local database for preservation. Through the process of fault localization, \tool was able to identify a list of potential fault locations, prioritizing src/epoch.rs:1053:43 as the most likely candidate—a determination that precisely matched the location of the eventual patch. Following this, the phase of patch generation commenced, during which \tool successfully generated a total of four patches for the top-ranked location. The patch we ultimately selected to commit, ranked top-1, employs the "Insert Range Checker" pattern, which is detailed in Section~\ref{subsec:pattern_mining} and is illustrated below:

% out-of-bounds: https://github.com/nyx-space/hifitime/pull/284
\begin{listing}[h]
\begin{minted}[linenos=false,
fontsize=\small]{diff}
+ if prev_idx > end_idx {
+    return Err(Errors::ParseError(ParsingErrors::ISO8601));
+ }
match lexical_core::parse(s[prev_idx..end_idx].as_bytes()) {
\end{minted}
\caption{A patch for a Rust crate that fixes panic caused by index out of bounds.}
\label{lst:rq4-1}
\end{listing}

The prominent ranking of the patch can be attributed to its direct relevance to the panic situation encountered. The Insert Range Checker pattern, which \tool employs, specifically targets index or range expressions within Rust code. In this instance, the fault was identified within a match expression; however, a closer inspection through iterative analysis of the AST revealed that this match expression included a range expression, making it a suitable candidate for the applied pattern. This rationale holds true for Listing~\ref{lst:rq4-2} as well, where the top-ranked patch was similarly adopted. For this instance, \tool leveraged the Insert Match Unwrapper pattern, designed to tackle issues associated with the use of unwrap. Highlighted in the code snippet below is the precise fault location: a let statement initializing an expression through a method call that employs unwrap. Moreover, the efficacy of the patch extends beyond merely addressing the panic; it also successfully passes all regression tests, further validating its correctness and compatibility with the existing codebase. Additionally, the accuracy and precision in fault localization play a significant role in elevating the patch's ranking. 

% unwrap: https://github.com/nyx-space/hifitime/pull/285
\begin{listing}[h]
\begin{minted}[linenos=false,
fontsize=\small]{diff}
- let mut cur_item = self.items[cur_item_idx].unwrap();
+ let mut cur_item =  match self.items[cur_item_idx] {
+     Some(item) => item,
+     None => return Err(Errors::ParseError
+                       (ParsingErrors::UnknownFormat)),
\end{minted}
\caption{A patch for a Rust crate that fixes panic caused by unwrap on None and other invalid value.}
\label{lst:rq4-2}
\end{listing}

The description on fix patches by \tool plays a crucial role in the real-world software development workflow, as the process of fixing issues extends beyond merely generating output—it necessitates active engagement with developers, for whom the interpretability of code is essential. When we submitted the pull requests for Listings~\ref{lst:rq4-1} and \ref{lst:rq4-2}, we capitalized on the insights gained from the pattern descriptions. For instance, we elucidated the specific cause of the error in our proposed fixes: highlighting that the panic was triggered by the condition prev\_idx > end\_idx, rather than the more generic begin <= end error message cited in the panic alert. This detailed explanation, provided in our patch descriptions, not only clarifies the rationale behind our fixes but also facilitates a deeper understanding and appreciation of the proposed changes among the reviewing developers. Such comprehensive communication is instrumental in fostering a collaborative and informed review process, ultimately enhancing the quality and acceptance of contributions to the codebase. 

During our interactions with developers, we gleaned valuable feedback that was instrumental in refining our approach. One particularly enlightening exchange occurred with a maintainer regarding the Mutate Binary Operator pattern. This pattern, designed to accommodate a range of binary operators, offers various mutation options, such as transitioning to either saturating or checked method calls. Initially, we submitted a patch utilizing a saturating call, which was ranked top-1. However, through detailed discussions, we pivoted to a checked method call based on the maintainer's input. The maintainer articulated his design philosophy on handling arithmetic overflow errors as follows:

\textsf{...we want to fail early and give an indication of what has happened, and prevent the user from thinking that the date they provided was correct...}

Guided by this feedback, we revised our patch to incorporate a checked method call with explicit error handling, which was also integrated into our collection of patches. This adaptation underscored a significant challenge for \tool: aligning with the authentic design intentions of software projects. We anticipate that offering a top-5 recommendation list could mitigate this challenge by presenting users with a spectrum of potential solutions. The discussion also underscores the importance of meaningful collaboration between tool developers and code maintainers. Such interactions are pivotal for advancing APR research, enhancing the practical impact, and facilitating its adoption in real-world software development scenarios.

==> sec/result.tex <==
In this section, we present the experiment results on automatically fixing panic bugs and then analyze the effectiveness and efficiency of our proposed tool \tool.



\subsection{Answer to RQ1: Fault Localization} \label{subsec:rq1}
To comprehensively assess the effectiveness of fault localization through various techniques, we employ three granularity levels for locating panics: file, statement, and expression levels. 
As illustrated in Table~\ref{tab:rq1}, the localization accuracy of \tool at all three granularities is higher than the other baselines, which indicates the effectiveness of \tool.
In addition, all methods perform better on the small-scale dataset compared with the large-scale dataset. 
This result is as expected, because on large-scale projects, the stack unfolding information could be more complex and harder to analyze the dependency for fault localization.
The effectiveness of the random method is relatively close to \tool, especially on small-scale datasets and top-5 prediction results, which suggests that if the localization is in the stack-expanded list, random selection can be effective, but as soon as in-depth dependency analyses are required on large-scale dataset, the random method fails outright.
The similarity-based selection techniques are the least effective in terms of fine-grained localization accuracy, implying that relying on natural language alone does not accurately capture the semantic information of complex practical code, resulting in low localization accuracy.

As for comparing with LLM-based approaches, the localization accuracy of ChatGPT4 is basically the same for single and multi-round conversations due to a limited understanding of an entire Rust project. This limitation is evident in the significant drop in success rate as the size of the Rust project increases. 
Throughout our experiments, we observed instances where ChatGPT failed to parse files accurately, providing only general suggestions that are impractical for effective fault localization. These observations highlight the inconsistency and limitations of relying on LLMs for accurate bug localization in complex codebases.



For spectrum-based methods, both Ochiai and Tarantula methods exhibited low accuracy, particularly within larger datasets, where Ochiai, for instance, showed zero accuracy in the top-1 ranking across all levels. 
This may because that panic bugs in Rust program constitute a unique category of errors, usually not originating from traditional issues in loops or conditional logic. The unit test cases within each crate aim to validate logical functionality, thus testing pass and fail conditions that may not align with detecting panic-related bugs. This mismatch could reduce the effectiveness of spectrum-based techniques. 
In addition, facing with real-world and large-scale programs that contain thousands of lines code, applying spectrum-based techniques incurs considerable time overheads, further limiting their practicality. 
% In fact, the time consumption of these spectrum-based methods is significantly higher compared to our approach. 
For example, calculating the spectrum score for a project could takes more than 3 hours in average for the large-scale dataset, while \tool takes about 1 minute in average. 

\begin{table}[htbp]
\centering
\caption{The correctness of tools on \dataset datasets, with different granularities of error localization.}
\vspace{-5pt}
\label{tab:rq1}
\scriptsize
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{cc|ccc|ccc||ccc}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Tool}}} & \multicolumn{3}{c|}{\textbf{\dataset-Small (61)}}     & \multicolumn{3}{c||}{\textbf{\dataset-Large (41)}}   & \multicolumn{3}{c}{\textbf{Total (102)}}    \\ %\cline{3-11} 
&& \textbf{File}  & \textbf{Stmt}  & \textbf{Expr}  & \textbf{File}  & \textbf{Stmt}  & \textbf{Expr}  & \textbf{File}  & \textbf{Stmt} & \textbf{Expr}  \\ \midrule
\multirow{8}{*} {Top-1} & panic        & 41 (67.2\%) & 30 (49.2\%) & 30 (49.2\%) & 22 (53.7\%) & 10 (24.4\%) & 10 (24.4\%) & 63 (61.8\%) & 40 (39.2\%) & 40 (39.2\%) \\ 
& random       & 33 (54.1\%) & 14 (23.0\%)  & 13 (21.3\%)  & 14 (34.1\%) & 7 (17.1\%)  & 6 (14.6\%) & 47 (46.1\%) & 21 (20.6\%) & 19 (18.6\%) \\ 
& similarity          & 13 (21.3\%)  & 0 (0\%)     & 0 (0\%)     & 7 (17.1\%)  & 1 (2.4\%)   & 0 (0\%)   & 20 (19.6\%) & 1 (1.0\%)   & 0 (0\%)   \\ \cline{2-11}
& Ochiai  & 0 (0\%) & 0 (0\%)  & 0 (0\%)  & 0 (0\%) & 0 (0\%)  & 0 (0\%) & 0 (0\%) & 0 (0\%) & 0 (0\%) \\ 
& Tarantula  & 1 (1.6\%) & 1 (1.6\%)  & 1 (1.6\%)  & 0 (0\%) & 0 (0\%)  & 0 (0\%) & 1 (1.0\%) & 1 (1.0\%) & 1 (1.0\%) \\ \cline{2-11}
& GPT-4        & 42 (68.9\%) & 28 (45.9\%) & 19 (31.1\%) & 10 (24.4\%)  & 4 (9.8\%)  & 3 (7.3\%) & 52 (51.0\%) & 32 (31.4\%) & 22 (21.6\%) \\ 
& GPT4-multi   & 43 (70.5\%) & 28 (45.9\%) & 19 (31.1\%) & 10 (24.4\%)  & 4 (9.8\%)  & 3 (7.3\%) & 53 (52.0\%) & 32 (31.4\%) & 22 (21.6\%) \\ 
&\textbf{\tool}  & \textbf{45 (73.8\%)} & \textbf{33 (54.1\%)} & \textbf{32 (52.5\%)} & \textbf{22 (53.7\%)} & \textbf{13 (31.7\%)} & \textbf{13 (31.7\%)} & \textbf{67 (65.7\%)} & \textbf{46 (45.1\%)} & \textbf{45 (44.1\%)} \\ \midrule
\multirow{7}{*} {Top-3} & random       & 46 (75.4\%) & 29 (47.5\%) & 29 (47.5\%) & 17 (41.5\%) & 8 (19.5\%)  & 8 (19.5\%) & 63 (61.8\%) & 37 (36.3\%) & 37 (36.3\%) \\ 
& similarity          & 21 (34.4\%)  & 1 (1.6\%)     & 1 (1.6\%)     & 10 (24.4\%)  & 1 (2.4\%)   & 0 (0\%)   & 31 (30.4\%) & 2 (2.0\%) & 1 (1.0\%)   \\ \cline{2-11}
& Ochiai  & 3 (5.0\%) & 3 (5.0\%)  & 3 (5.0\%)  & 0 (0\%) & 0 (0\%)  & 0 (0\%) & 3 (2.9\%) & 3 (2.9\%) & 3 (2.9\%) \\ 
& Tarantula  & 2 (3.3\%) & 2 (3.3\%)  & 2 (3.3\%)  & 0 (0\%) & 0 (0\%)  & 0 (0\%) & 2 (2.0\%) & 2 (2.0\%) & 2 (2.0\%) \\ \cline{2-11}
& GPT-4        & 43 (70.5\%) & 29 (47.5\%) & 20 (32.8\%) & 12 (29.3\%)  & 4 (9.8\%)  & 3 (7.3\%) & 55 (53.9\%) & 33 (32.4\%) & 23 (22.5\%) \\ 
& GPT4-multi   & 44 (72.1\%) & 29 (47.5\%) & 20 (32.8\%) & 12 (29.3\%)  & 4 (9.8\%)  & 3 (7.3\%) & 56 (54.9\%) & 33 (32.4\%) & 23 (22.5\%) \\ 
&\textbf{\tool}  & \textbf{49 (80.3\%)} & \textbf{38 (62.3\%)} & \textbf{37 (60.7\%)} & \textbf{28 (68.3\%)} & \textbf{19 (46.3\%)} & \textbf{18 (43.9\%)} & \textbf{77 (75.5\%)} & \textbf{57 (55.9\%)} & \textbf{55 (53.9\%)} \\ \midrule
\multirow{7}{*} {Top-5} & random       & 48 (78.7\%) & 33 (54.1\%) & 33 (54.1\%) & 22 (53.7\%) & 13 (31.7\%) & 12 (29.3\%) & 70 (68.6\%) & 46 (45.1\%) & 45 (44.1\%) \\ 
& similarity          & 25 (41.0\%)  & 1 (1.6\%)     & 1 (1.6\%)     & 13 (31.7\%) & 1 (2.4\%)   & 0 (0\%)  & 38 (37.3\%) & 2 (2.0\%) & 1 (1.0\%)   \\\cline{2-11}
& Ochiai  & 9 (14.8\%) & 9 (14.8\%)  & 9 (14.8\%)  & 0 (0\%) & 0 (0\%)  & 0 (0\%) & 9 (8.8\%) & 9 (8.8\%) & 9 (8.8\%) \\ 
& Tarantula  & 6 (9.8\%) & 6 (9.8\%)  & 6 (9.8\%)  & 1 (2.4\%) & 1 (2.4\%)  & 1 (2.4\%) & 7 (6.9\%) & 7 (6.9\%) & 7 (6.9\%) \\ \cline{2-11}
& GPT-4        & 46 (75.4\%) & 30 (49.2\%) & 21 (34.4\%) & 14 (34.1\%) & 4 (9.8\%)  & 3 (7.3\%) & 60 (58.8\%) & 34 (33.3\%) & 24 (23.5\%) \\
& GPT4-multi   & 47 (77.0\%) & 30 (49.2\%) & 21 (34.4\%) & 14 (34.1\%) & 4 (9.8\%)  & 3 (7.3\%) & 61 (59.8\%) & 34 (33.3\%) & 24 (23.5\%) \\ 
&\textbf{\tool}  & \textbf{49 (80.3\%)} & \textbf{38 (62.3\%)} & \textbf{37 (60.7\%)} & \textbf{29 (70.7\%)} & \textbf{20 (48.8\%)} & \textbf{19 (46.3\%)} & \textbf{78 (76.5\%)} & \textbf{58 (56.9\%)} & \textbf{56 (54.9\%)} \\ \bottomrule
\end{tabular}}
%\vspace{-10pt}
\end{table}

%%%%%%% synthetic dataset %%%%%%%%%
% As for the synthetic dataset, except for the natural language similarity technique, the accuracy of other methods is very close to each other, all of which are around $95\%$.
% % On the one hand, the code in the synthetic dataset is small in size, typically just 2 or 3 files with about 20 lines of code, thus almost all methods can locate the exact file and statement with relatively high accuracy.
% % On the other hand, 
% Although in terms of localization accuracy, \tool has $1$ fewer correct localization than ChatGPT, we believe that this belongs to an overfitting problem of other methods.
% We consider that panics caused by assertion failures are intended by the program and are not bugs nor do they need to be fixed, therefore, for such a case in the synthetic data, \tool does not output the corresponding localization information, whereas other techniques, including ChatGPT, localize the assertion, which leads to overfitting problems~\cite{ye2022overfit, xin2017overfit}.
% To summarize, compared to existing techniques, \tool achieves better localization accuracy on large-scale real projects, and can effectively avoid overfitting problems.
%%%%%%% synthetic dataset %%%%%%%%%



% \vspace{-6pt}
\subsection{Answer to RQ2: Fixing Effectiveness}
% We evaluate the fixing effectiveness of \tool and baseline approaches.
Because there is no existing APR tool for Rust panic bugs, we focus on comparison the fixing effectiveness with ChatGPT-4.
% Specifically, regarding the real dataset, we conduct separate assessments for various metrics: the percentage of fixes that exactly match the actual fixes implemented, the percentage of fixes that fix panic and pass all regression tests, which are regarded as correct, and the percentage of fixes that fix panic but fail to fully pass the regression tests, classified as plausible.
% For the synthetic dataset, we only report the percentage of same and plausible fixes, because the semantics are simple and there are no regression test suites.
The evaluation results are shown in Table~\ref{tab:rq2.1}.
Overall, we can conclude that \tool significantly surpasses the performance of automated repairs conducted by GPT-4. 
Notably, within the large-scale dataset, GPT-4 fails to generate any viable patches, the reason of which is closely tied to GPT-4's challenges with fault localization, as elaborated in Section~\ref{subsec:rq1}. 
Moreover, we find that LLM-based methods frequently overlooks the code context when generating patches, resulting in the generated program failing to compile instead.
For example, it may attempt to resolve panics by altering a method's return type directly or by incorporating new logic, which results in both compilation and semantic errors.


\begin{table}[htbp]
\centering
\footnotesize
\caption{The number of eliminated/plausible/correct patches of different tools on \dataset.} 
\vspace{-5pt}
\label{tab:rq2.1}
\setlength{\tabcolsep}{0.6mm}{ 
\begin{tabular}{cc|cc|cc|cc|cc|cc|cc||cc|cc|cc}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Tool}}} & \multicolumn{6}{c|}{\textbf{\dataset-Small (61)}}                                         & \multicolumn{6}{c||}{\textbf{\dataset-Large (41)}}          & \multicolumn{6}{c}{\textbf{Total (102)}}                \\ %\cline{3-8} 
&   & \multicolumn{2}{c|}{\textbf{Eliminated}} & \multicolumn{2}{c|}{\textbf{Plausible}}      & \multicolumn{2}{c|}{\textbf{Correct}}       & \multicolumn{2}{c|}{\textbf{Eliminated}} & \multicolumn{2}{c|}{\textbf{Plausible}}   & \multicolumn{2}{c||}{\textbf{Correct}}  & \multicolumn{2}{c|}{\textbf{Eliminated}} & \multicolumn{2}{c|}{\textbf{Plausible}}  & \multicolumn{2}{c}{\textbf{Correct}} \\ \midrule
%\multirow{3}{*} {Top-1}
\multirow{3}{*}{\begin{sideways}Top-1\end{sideways}} 
& GPT-4          
& 6 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%  & 6 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\% & 0  & \cellcolor[rgb]{ .930,  .930,  .930}0\%  

& 0  & \cellcolor[rgb]{ .930,  .930,  .930}0\%    & 0 & \cellcolor[rgb]{ .930,  .930,  .930}0\%  & 0 & \cellcolor[rgb]{ .930,  .930,  .930}0\%

& 6 & \cellcolor[rgb]{ .930,  .930,  .930}5.9\%   & 6 & \cellcolor[rgb]{ .930,  .930,  .930}5.9\% & 0 & \cellcolor[rgb]{ .930,  .930,  .930}0\% \\
& GPT4-multi      
& 8 & \cellcolor[rgb]{ .930,  .930,  .930}13.1\%  & 8 & \cellcolor[rgb]{ .930,  .930,  .930}13.1\%    & 0  & \cellcolor[rgb]{ .930,  .930,  .930}0\%   
& 0 & \cellcolor[rgb]{ .930,  .930,  .930}0\%    & 0 & \cellcolor[rgb]{ .930,  .930,  .930}0\%    
& 0  & \cellcolor[rgb]{ .930,  .930,  .930}0\% 

& 8 & \cellcolor[rgb]{ .930,  .930,  .930}7.8\%   & 8 & \cellcolor[rgb]{ .930,  .930,  .930}7.8\% & 0  & \cellcolor[rgb]{ .930,  .930,  .930}0\% \\
& \textbf{\tool}   
& \textbf{29} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{47.5\%}  & \textbf{19} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{31.1\%}  & \textbf{4} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{6.6\%}
& \textbf{10} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{24.4\%} & \textbf{7} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{17.1\%} & \textbf{4} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{9.8\%}
& \textbf{39} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{38.2\%} & \textbf{26} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{25.5\%} & \textbf{8} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{7.8\%}\\ \midrule
% \multirow{3}{*}{Top-3}
\multirow{3}{*}{\begin{sideways}Top-3\end{sideways}} 
& GPT-4         
& 6 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%  & 6 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\% & 1 & \cellcolor[rgb]{ .930,  .930,  .930}1.6\% 
&0 & \cellcolor[rgb]{ .930,  .930,  .930}0\%    & 0 &\cellcolor[rgb]{ .930,  .930,  .930}0\% & 0 &\cellcolor[rgb]{ .930,  .930,  .930}0\% 
& 6 & \cellcolor[rgb]{ .930,  .930,  .930}5.9\% & 6 & \cellcolor[rgb]{ .930,  .930,  .930}5.9\% & 1 &\cellcolor[rgb]{ .930,  .930,  .930}1.0\% \\
& GPT4-multi   
& 8 & \cellcolor[rgb]{ .930,  .930,  .930}13.1\%  & 8 & \cellcolor[rgb]{ .930,  .930,  .930}13.1\%   & 1 & \cellcolor[rgb]{ .930,  .930,  .930}1.6\%
& 0 & \cellcolor[rgb]{ .930,  .930,  .930}0\%    & 0 & \cellcolor[rgb]{ .930,  .930,  .930}0\% & 0 &\cellcolor[rgb]{ .930,  .930,  .930}0\% 
& 8 & \cellcolor[rgb]{ .930,  .930,  .930}7.8\% & 8 & \cellcolor[rgb]{ .930,  .930,  .930}7.8\% & 1 &\cellcolor[rgb]{ .930,  .930,  .930}1.0\%\\
& \textbf{\tool} 
& \textbf{32} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{52.5\%} & \textbf{23} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{37.7\%} & \textbf{12} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{19.7\%} 
& \textbf{13} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{31.7\%} & \textbf{10} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{24.4\%} & \textbf{7} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{17.1\%} 
& \textbf{45} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{41.1\%} & \textbf{33} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{32.4\%} & \textbf{19} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{18.6\%} \\ \midrule
% \multirow{3}{*}{Top-5}
\multirow{3}{*}{\begin{sideways}Top-5\end{sideways}} 
& GPT-4         
& 7 & \cellcolor[rgb]{ .930,  .930,  .930}11.5\%  & 7 & \cellcolor[rgb]{ .930,  .930,  .930}11.5\%  & 1 & \cellcolor[rgb]{ .930,  .930,  .930}1.6\%  
& 0  & \cellcolor[rgb]{ .930,  .930,  .930}0\%    & 0 & \cellcolor[rgb]{ .930,  .930,  .930}0\% & 0 & \cellcolor[rgb]{ .930,  .930,  .930}0\% 
& 7 & \cellcolor[rgb]{ .930,  .930,  .930}6.9\% & 7 & \cellcolor[rgb]{ .930,  .930,  .930}6.9\% & 1 & \cellcolor[rgb]{ .930,  .930,  .930}1.0\% \\
& GPT4-multi   
& 9 & \cellcolor[rgb]{ .930,  .930,  .930}14.8\%  & 9 & \cellcolor[rgb]{ .930,  .930,  .930}14.8\%   & 1 & \cellcolor[rgb]{ .930,  .930,  .930}1.6\% 
& 0 & \cellcolor[rgb]{ .930,  .930,  .930}0\%    & 0 & \cellcolor[rgb]{ .930,  .930,  .930}0\% & 0 & \cellcolor[rgb]{ .930,  .930,  .930}0\% 
& 9 & \cellcolor[rgb]{ .930,  .930,  .930}8.8\% & 9 & \cellcolor[rgb]{ .930,  .930,  .930}8.8\% & 1 & \cellcolor[rgb]{ .930,  .930,  .930}1.0\% \\
& \textbf{\tool} 
& \textbf{35} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{57.4\%} & \textbf{25} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{41.0\%} & \textbf{12} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{19.7\%} 
& \textbf{14} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{34.1\%} & \textbf{10} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{24.4\%} & \textbf{7} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{17.1\%} 
& \textbf{49} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{48.0\%} & \textbf{35} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{34.3\%} & \textbf{19} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{18.6\%} \\ 
\bottomrule
\end{tabular}}
% \vspace{-10pt}
\end{table}


% \liu{@yb:Add the description of Table VII here.}
As shown in Table~\ref{tab:rq2.2}, even with perfect location information, \tool consistently outperforms GPT-4. 
This indicates that \tool's patch generation capability is superior to that of GPT-4, even after multiple iterations. 
Compared with the results in Table~\ref{tab:rq2.1}, \tool only slightly improves its fixing effectiveness with perfect location information. While it does generate new plausible or correct patches, it sometimes fails to recreate some of its previous patches without perfect locations. 
This is because some patches were applied at related but different locations, such as within a method call hierarchy, and still effectively fixed the issue.
However, the provided location may interfere with the selection of fix patterns.
As for ChatGPT, when provided with exact fault locations, it can generate a few effective patches for large datasets, a stark improvement over its complete failure without precise locations. This further underscores the deficiency in GPT-4's fault localization capabilities.


\begin{table}[htbp]
\centering
\footnotesize
\caption{The number of eliminated/plausible/correct patches of different tools on \dataset with perfect locations.} 
\label{tab:perfect}
\vspace{-5pt}
\label{tab:rq2.2}
\setlength{\tabcolsep}{0.6mm}{ 
\begin{tabular}{cc|cc|cc|cc|cc|cc|cc||cc|cc|cc}
\toprule
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Tool}}} & \multicolumn{6}{c|}{\textbf{\dataset-Small (61)}}                                         & \multicolumn{6}{c||}{\textbf{\dataset-Large (41)}}          & \multicolumn{6}{c}{\textbf{Total (102)}}                \\ %\cline{3-8} 
&   & \multicolumn{2}{c|}{\textbf{Eliminated}} & \multicolumn{2}{c|}{\textbf{Plausible}}      & \multicolumn{2}{c|}{\textbf{Correct}}       & \multicolumn{2}{c|}{\textbf{Eliminated}} & \multicolumn{2}{c|}{\textbf{Plausible}}   & \multicolumn{2}{c||}{\textbf{Correct}}  & \multicolumn{2}{c|}{\textbf{Eliminated}} & \multicolumn{2}{c|}{\textbf{Plausible}}  & \multicolumn{2}{c}{\textbf{Correct}} \\ \midrule
%\multirow{3}{*} {Top-1}
\multirow{3}{*}{\begin{sideways}Top-1\end{sideways}} 
& GPT-4          
& 6 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%  & 4 & \cellcolor[rgb]{ .930,  .930,  .930}6.6\% & 4 & \cellcolor[rgb]{ .930,  .930,  .930}6.6\%
& 3  & \cellcolor[rgb]{ .930,  .930,  .930}7.3\%    & 3 & \cellcolor[rgb]{ .930,  .930,  .930}7.3\%    & 3 & \cellcolor[rgb]{ .930,  .930,  .930}7.3\%    
& 9 & \cellcolor[rgb]{ .930,  .930,  .930}8.8\%   & 7 & \cellcolor[rgb]{ .930,  .930,  .930}6.9\% & 7 & \cellcolor[rgb]{ .930,  .930,  .930}6.9\% \\
& GPT4-multi      
& 6 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%  & 4 & \cellcolor[rgb]{ .930,  .930,  .930}6.6\% & 4 & \cellcolor[rgb]{ .930,  .930,  .930}6.6\%
& 3 & \cellcolor[rgb]{ .930,  .930,  .930}7.3\%    & 3 & \cellcolor[rgb]{ .930,  .930,  .930}7.3\%    & 3 & \cellcolor[rgb]{ .930,  .930,  .930}7.3\%    
& 9 & \cellcolor[rgb]{ .930,  .930,  .930}8.8\%   & 7 & \cellcolor[rgb]{ .930,  .930,  .930}6.9\% & 7 & \cellcolor[rgb]{ .930,  .930,  .930}6.9\% \\
& \textbf{\tool}   
& \textbf{33} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{54.1\%}  & \textbf{24} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{39.3\%} & 7 & \cellcolor[rgb]{ .930,  .930,  .930}11.5\%  
& \textbf{10} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{24.4\%} & \textbf{7} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{17.1\%} & 4 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\% 
& \textbf{43} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{42.2\%} & \textbf{31} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{30.4\%} & 11 & \cellcolor[rgb]{ .930,  .930,  .930}10.8\% \\ \midrule
% \multirow{3}{*}{Top-3}
\multirow{3}{*}{\begin{sideways}Top-3\end{sideways}} 
& GPT-4         
& 6 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%  & 5 & \cellcolor[rgb]{ .930,  .930,  .930}8.2\% & 4 & \cellcolor[rgb]{ .930,  .930,  .930}6.6\% 
&3 & \cellcolor[rgb]{ .930,  .930,  .930}7.3\%    & 3 &\cellcolor[rgb]{ .930,  .930,  .930}7.3\%  & 3 &\cellcolor[rgb]{ .930,  .930,  .930}7.3\%
& 9 & \cellcolor[rgb]{ .930,  .930,  .930}8.8\% & 8 & \cellcolor[rgb]{ .930,  .930,  .930}7.8\%  & 7 &\cellcolor[rgb]{ .930,  .930,  .930}6.9\%\\
& GPT4-multi   
& 6 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%  & 5 & \cellcolor[rgb]{ .930,  .930,  .930}8.2\%  & 4 &\cellcolor[rgb]{ .930,  .930,  .930}6.6\%
& 3 & \cellcolor[rgb]{ .930,  .930,  .930}7.3\%    & 3 & \cellcolor[rgb]{ .930,  .930,  .930}7.3\%     & 3 &\cellcolor[rgb]{ .930,  .930,  .930}7.3\%
& 9 & \cellcolor[rgb]{ .930,  .930,  .930}8.8\% & 8 & \cellcolor[rgb]{ .930,  .930,  .930}7.8\%  & 7 &\cellcolor[rgb]{ .930,  .930,  .930}6.9\%\\
& \textbf{\tool} 
& \textbf{36} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{59.0\%} & \textbf{27} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{44.3\%}  & 15 &\cellcolor[rgb]{ .930,  .930,  .930}24.6\%
& \textbf{13} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{31.7\%} & \textbf{11} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{26.8\%}  & 9 &\cellcolor[rgb]{ .930,  .930,  .930}22.0\%
& \textbf{49} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{48.0\%} & \textbf{38} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{37.3\%}  & 24 &\cellcolor[rgb]{ .930,  .930,  .930}23.5\%\\ \midrule
% \multirow{3}{*}{Top-5}
\multirow{3}{*}{\begin{sideways}Top-5\end{sideways}} 
& GPT-4         
& 6 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%  & 5 & \cellcolor[rgb]{ .930,  .930,  .930}8.2\% & 4 & \cellcolor[rgb]{ .930,  .930,  .930}6.6\% 
& 4  & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%    & 4 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%    & 4 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%
& 10 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\% & 9 & \cellcolor[rgb]{ .930,  .930,  .930}8.8\% & 8 & \cellcolor[rgb]{ .930,  .930,  .930}7.8\%\\
& GPT4-multi   
& 6 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%  & 5 & \cellcolor[rgb]{ .930,  .930,  .930}8.2\% & 4 & \cellcolor[rgb]{ .930,  .930,  .930}6.6\%
& 4 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%    & 4 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%    & 4 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\%
& 10 & \cellcolor[rgb]{ .930,  .930,  .930}9.8\% & 9 & \cellcolor[rgb]{ .930,  .930,  .930}8.8\% & 8 & \cellcolor[rgb]{ .930,  .930,  .930}7.8\%\\
& \textbf{\tool} 
& \textbf{36} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{59.0\%} & \textbf{27} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{44.3\%} & 15 &\cellcolor[rgb]{ .930,  .930,  .930}24.6\%
& \textbf{13} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{31.7\%} & \textbf{11} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{26.8\%} & 9 &\cellcolor[rgb]{ .930,  .930,  .930}22.0\%
& \textbf{49} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{48.0\%} & \textbf{38} & \cellcolor[rgb]{ .930,  .930,  .930}\textbf{37.3\%} & 24 &\cellcolor[rgb]{ .930,  .930,  .930}23.5\%\\ 
\bottomrule
\end{tabular}}
\vspace{-10pt}
\end{table}


Regarding to the plausible and panic-eliminated patches, we believe that, when coupled with the textual interpretations derived from our mined patterns, panic-eliminated patches can aid developers repair their program efficiently.
This is because the failure of some patches to pass the regression tests may be attributed to additional logic after the patch is applied, which is beyond APR's capabilities.
% For instance, one unsuccessful patch generated by \tool involved the addition of an \texttt{as\_bytes()} method call to a variable for its return value, mirroring the developers' own solution. 
% This modification necessitated altering the return type of the variable, resulting in issues not directly related to the original bug, a phenomenon identified in prior research~\cite{yoo2012regression, huang2023survey}. 
% Nonetheless, the patches for panic bugs provided by \tool are fundamentally correct.
Such plausible fixes, with minimal manual oversight, can be comprehensively resolved, thereby reducing the developers' burden in understanding panic bugs and evaluating alternative functions.





%\vspace{-6pt}
\subsection{Answer to RQ3: Efficiency}
% Table~\ref{tab:rq3} reports the efficiency of \tool compared to the duration required for manual fixes. 
% Besides, 


Fig~\ref{fig:rq3} and Table~\ref{tab:rq3} show the distribution of time spent on \tool and manual fixes.
On average, \tool requires about one minute to repair panics, whereas manual repairs can take days.
An interesting observation is that the average time of both \tool and manual repair are generally longer for smaller datasets. 
For \tool, this extended time is mainly due to the large test suites in some libraries, which lengthen the validation process. 
In terms of manual repairs, one notable case involved a panic bug that took over two years to fix, largely due to delayed maintenance by developers, resulting in a notably prolonged repair time for a smaller dataset.



% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.95\linewidth]{fig/rq3_boxplot.pdf}
%     \vspace{-10pt}
%     \caption{Experiment results of efficiency.}
%     \label{fig:rq3}
%     \vspace{-10pt}
% \end{figure}

\begin{wrapfigure}{r}{6cm}%靠文字内容的右侧
\centering
% \vspace{-15pt}
  \includegraphics[width=0.95\linewidth]{fig/rq3_boxplot.pdf}
  \vspace{-15pt}
  \caption{Experiment results of efficiency.}
  \vspace{-15pt}
  \label{fig:rq3}
\end{wrapfigure}



In examining real-world PRs, we found a few key factors that potentially affect the bug-fixing time.
Developers often spend several days discussing issues due to the need to comprehend error messages, understand collaborators' code, and locate faults. 
Conversely, \tool provides detailed explanations with fix patches to streamline the review process and improve developer understanding. 
Additionally, maintainers sometimes request multiple revisions of a submitted fix, requiring different approaches and thus increasing time and effort. 
\tool addresses this by generating a range of patches, ranking them based on confidence scores and validation results, thus offering a prioritized patch list.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
\centering
\small
\caption{Time consuming for \tool and actual fixes.} 
\vspace{-5pt}
\label{tab:rq3}
\begin{tabular}{ccccc}
\toprule
\textbf{Datasets}    & \textbf{Approaches}   & \textbf{Min} & \textbf{Max}     & \textbf{Avg.}  \\ \midrule
\textbf{\dataset-} & \tool & 0.51s   & 588.72s     & 65.77s  \\
\textbf{Small} & \cellcolor[rgb]{ .930,  .930,  .930}Actual     & \cellcolor[rgb]{ .930,  .930,  .930}0.52h    & \cellcolor[rgb]{ .930,  .930,  .930}807 days & \cellcolor[rgb]{ .930,  .930,  .930}76 days \\ \midrule
\textbf{\dataset-} & \tool & 0.34s  & 425.32s     & 61.29s      \\
\textbf{Large} & \cellcolor[rgb]{ .930,  .930,  .930}Actual      & \cellcolor[rgb]{ .930,  .930,  .930}0.42h   & \cellcolor[rgb]{ .930,  .930,  .930}236 days   & \cellcolor[rgb]{ .930,  .930,  .930}44 days \\
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Answer to RQ4: Case Study} \label{subsec:ans_rq4}

% \liu{Let's consider adding a table that shows how many open/closed issues we collected on 10 crates (not in \dataset), and the corresponding fixes.}
% 1. 4 crates with hundreds and even thousands of stars
% 2. open and closed issues - unresloved and resolved issues
% 3. open: apply to it -> developer approve -> merge + still
% 4. close: apply to it without perfect location -> apply TF-IDF to calculate similarity -> over 0.75 and fix panic -> similar



% To demonstrate the practical effects of \tool on large-scale Rust programs, we apply it to open and closed panic-related issues within real Rust projects on GitHub. 
% All of the selected crates are included in \dataset, and we employ \tool to generate fix patches. 
% For open issues, the generated patches are submitted to pull requests (PRs), and we track whether they are confirmed and merged by developers. 
% We use TF-IDF~\cite{sparck1972statistical} to calculate the similarity between the generated patches and the official ones. If the similarity score exceeds $0.75$, and the panic is fixed with the regression test passed, we consider the \tool-generated patch to be similar to the official patch. 


The overall evaluation results on real-world projects are presented in Table~\ref{tab:rq4}, showing that \tool successfully resolved 28 of 41 open issues with varied root causes, with all patches merged by developers. 
% These causes encompass arithmetic overflow, index-out-of-bounds errors, and unwrapping on None or invalid values, among others. 
% Besides, \tool has also generated some plausible patches that eliminated the panic, necessitating manual inspection and slight adjustments. 
As for unsuccessful fixes, some patches were plausible; they removed the panic but required further manual inspection and minor adjustments. 
% For some issues, no patch was generated due to the complexity of the panic's causes, suggesting the need to combine multiple repair patterns.
In terms of closed issues, \tool successfully generates 9 out of 22 patches that are similar to official patches.
The proportion is not very high, largely due to differences in their repair locations. For example, while the official approach might add a branch before the parameter call, \tool tends to insert it after creating the parameter. Nonetheless, both strategies achieve equivalent outcomes.




% Overall, \tool has successfully fixed 28 unique unresolved panic bugs with diverse root causes. 
% These root causes include arithmetic overflow, index-out-of-bounds errors, and unwrapping on None or invalid values, among others.
% Notably, \tool also generates some plausible patches that do not pass regression tests, which are not considered effective. 
% However, we believe these patches still offer significant value in the repair process. By identifying fault locations and providing initial patches, \tool aids developers in more easily understanding and addressing panic bugs. 
% In terms of resolved panic bugs, \tool successfully generates 9 patches that are similar to the official patches.

% To prove \tool's practical effect on large-scale Rust programs, we applied it to open and closed issues within real-world Rust projects open-sourced in GitHub. 
% We select four crates with hundreds or even thousands stars.
% As shown in Table~\ref{tab:rq4}, we collect panic-related issues for each crate, identifying unresolved panics from open issues and resolved panics from closed issues.

\begin{table}[htbp]
\centering
\small
\caption{Distribution of panics in real-world crates and fixing effectiveness of \tool.}
\vspace{-5pt}
\label{tab:rq4}
\setlength{\tabcolsep}{1.5mm}
%\begin{threeparttable}
\begin{tabular}{ccc|cc||cc}
\toprule
\multirow{2}{*}{\textbf{Crates}} & \multirow{2}{*}{\textbf{Stars}} & \multirow{2}{*}{\textbf{LoC}}& \multicolumn{2}{c||}{\textbf{Open issues}} & \multicolumn{2}{c}{\textbf{Closed issues}} \\
&   &  & \textbf{Total} & \textbf{Confirmed}      & \textbf{Total} & \textbf{Similar}    \\ \midrule
\textbf{hifitime}   & 315 & 10,762         & 28                & 21  & 0               & -          \\
\textbf{unicode-segmentation}  & 556 & 7,345            & 11                & 7   & 1               & 0     \\
\textbf{ratatui} & 9,086 & 41,534             & 1                 & 0      & 18              & 7  \\
\textbf{fancy-regex}  & 409 & 5,557       & 1                 & 0      & 3               & 2  \\ \midrule
\multicolumn{3}{c|}{\textbf{Total}}         & \textbf{41}                & \textbf{28}  & \textbf{22}              & \textbf{9}  \\ \bottomrule
\end{tabular}
% \begin{tablenotes}
%     \footnotesize
%     \item[1] The full name of this crate is: unicode-segmentation.
% \end{tablenotes}
%\end{threeparttable}
% \vspace{-10pt}
\end{table}

% For unresolved panics, we use \tool to generate patches and submit them for approval by the developers or maintainers. Once a patch is merged, it is deemed effective.
% For resolved panics, we also employ \tool to generate patches. We then use TF-IDF~\cite{} to calculate the similarity between these patches and the official ones. If the similarity score exceeds 0.75, and the panic is fixed with the regression test passed, we consider the \tool-generated patch to be similar to the official patch. 

% Overall, four unique panic bugs with diverse root causes, have been fixed by \tool without any human intervention.
% The covered root causes include arithmetic overflow, index-out-of-bounds, and unwrapping on None/invalid values.

% unresolved: overall 28/41 + include overflow+index+unwrap+... + some of them plausible though incorrect 
% Overall, \tool has successfully fixed 28 unique unresolved panic bugs with diverse root causes. 
% These root causes include arithmetic overflow, index-out-of-bounds errors, and unwrapping on None or invalid values, among others.
% Notably, \tool also generates some plausible patches that do not pass regression tests, which are not considered effective. 
% However, we believe these patches still offer significant value in the repair process. By identifying fault locations and providing initial patches, \tool aids developers in more easily understanding and addressing panic bugs. 
% In terms of resolved panic bugs, \tool successfully generates 9 patches that are similar to the official patches.


Below we illustrate some bug cases and their fixes.

\textbf{Bug Case1:}
Figure~\ref{fig:rq4} (a) shows the resolution of an arithmetic overflow error, which is a proposed patch of a closed issue for Rust crate ratatui~\cite{ratatui:online}.
% containing over $41$K lines of code and has more than $9$K stars.
% This panic bug is identified as resolved since it is collected from a closed issue.
% The panic error message is as follows:
% \textsf{
% thread 'main' panicked at 'begin <= end (21 <= 20) when slicing `94-11-05T08:15:34.0-:0`', /path/hifitime-3.8.2/src/epoch.rs:993:43
% }
Through fault localization, \tool succeeded in pinpointing a list of potential fault locations, prioritizing \texttt{src/layout.rs:233:20} as the top candidate, which aligns exactly with the actual fix.
% This demonstrates the effectiveness of our dependency analysis in accurately identifying the bug's source location, which plays an important role in guiding the automated repair process.
Then, \tool successfully generated 3 patches for this location. 
%\yb{3 patches for this location, 19 patches for all the locations, which one?}
In this case, the fault was identified within a struct filed expression; however, a closer inspection through iterative analysis revealed that this match expression included a binary expression, making it suitable for applying the \textit{Mutate Binary Operator} pattern. 
% The patch we ultimately selected to commit, ranked top-1, employs the \textit{Mutate Binary Operator} pattern, which is illustrated in detail in Section~\ref{subsec:pattern_mining}.
Finally, we calculate the similarity score between the generated patch and the official patch, obtaining a score of $0.95$, indicating the correctness. 

\begin{figure*}[tp]
    \centering
    \includegraphics[width=0.97\linewidth]{fig/case_study.pdf}
    \vspace{-5pt}
    \caption{Patches generated by \tool have fixed real-world issues.}
    \label{fig:rq4}
    \vspace{-10pt}
\end{figure*}

% % out-of-bounds: https://github.com/nyx-space/hifitime/pull/284
% \begin{listing}[h]
% \begin{minted}[linenos=false,
% fontsize=\footnotesize]{diff}
% + if prev_idx > end_idx {
% +    return Err(Errors::ParseError
% +        (ParsingErrors::ISO8601)); }
%   match lexical_core::parse(s[prev_idx..end_idx]
%                                     .as_bytes()) {
% \end{minted}
% \vspace{-6pt}
% \caption{A patch for the hifitime crate that fixes a panic bug caused by index out of bounds.}
% \label{lst:rq4-1}
% \end{listing}

% \begin{listing}[h]
% \begin{minted}[linenos=false,
% fontsize=\footnotesize]{diff}
% -   x: self.x + margin.horizontal,
% +   x: 0 + self.x.saturating_add(margin.horizontal),
%     y: self.y + margin.vertical,
% \end{minted}
% \vspace{-5pt}
% \caption{A generated patch for the crate ratatui that fixes a panic bug caused by arithmetic overflow.}
% \label{lst:rq4-1}
% \end{listing}


% unwrap: https://github.com/nyx-space/hifitime/pull/285
% \begin{listing}[h]
% \begin{minted}[linenos=false,
% fontsize=\footnotesize]{diff}
% - let mut cur_item = self.items[cur_item_idx].unwrap();
% + let mut cur_item = match self.items[cur_item_idx] {
% +   Some(item) => item,
% +   None => return Err(Errors::ParseError
% +                   (ParsingErrors::UnknownFormat)),
% + };
% \end{minted}
% \vspace{-5pt}
% \caption{A generated patch that fixes a panic bug in hifitime.}
% \label{lst:rq4-2}
% \end{listing}


% \vspace{-10pt}
\textbf{Bug Case 2:}
The patch illustrated in Figure~\ref{fig:rq4} (b), generated by \tool, serves as an example of addressing a panic bug that arises from unwrapping a None/invalid value. 
This bug comes from an open issue of Rust crate hifitime~\cite{hifitime:online}, and our patch has been merged by developers.
\tool employs the \textit{Insert Match Unwrapper} pattern, specifically designed to mitigate problems stemming from the misuse of unwrap. 
This approach transitions the unsafe usage of \texttt{unwarp()} to pattern matching, which results in returning an error message rather than triggering a panic error. 
Additionally, the patch created by \tool takes into consideration the variable types to ensure consistency with the code context, thereby guaranteeing that the modified program passes regression testing.




%%%%%%%%%%%%%%%
% In addition to improving code interpretability, the associated natural language interpretation accompanying the patches also plays an important role in real-world software development. 
% Our detailed explanations of the root causes in the pull requests, such as specifying that the panic was triggered by \texttt{prev\_idx} $>$ \texttt{end\_idx}, enhance understanding and facilitate developer review. 
% The subsequent verification and merging of our patches confirm their effectiveness and demonstrate \tool's practical utility in actual software applications.
%%%%%%%%%%%%%%%

% In addition to the generated patch, we believe the associated natural language interpretation also plays an important role in real-world software development, as it could improve code interpretability.
% When we submitted the pull requests for Listings~\ref{lst:rq4-1} and \ref{lst:rq4-2}, we capitalized on the insights gained from the pattern descriptions. 
% In particular, we elucidated the specific root causes, i.e., highlighting that the panic was triggered by the condition \texttt{prev\_idx} $>$ \texttt{end\_idx}, rather than the more generic \texttt{begin} $\geq$ \texttt{end} stated in error messages. 
% This detailed explanation, provided in our patch descriptions, not only clarifies the rationale behind our fixes but also facilitates a deeper understanding of the proposed changes among the reviewing developers. 
% Following verification, the developers confirmed our proposed localization, analysis, and patches which have all been merged into codebases. As a result, the patch is considered effective, further demonstrating the practical utility of \tool in real-world applications.

% Such comprehensive communication is instrumental in fostering a collaborative and informed review process, ultimately enhancing the quality and acceptance of contributions to the codebase. 

% During our interactions with developers, we gleaned valuable feedback that was instrumental in refining our approach. One particularly enlightening exchange occurred with a maintainer regarding the Mutate Binary Operator pattern. This pattern, designed to accommodate a range of binary operators, offers various mutation options, such as transitioning to either saturating or checked method calls. Initially, we submitted a patch utilizing a saturating call, which was ranked top-1. However, through detailed discussions, we pivoted to a checked method call based on the maintainer's input. The maintainer articulated his design philosophy on handling arithmetic overflow errors as follows:

% \textsf{...we want to fail early and give an indication of what has happened, and prevent the user from thinking that the date they provided was correct...}

% Guided by this feedback, we revised our patch to incorporate a checked method call with explicit error handling, which was also integrated into our collection of patches. This adaptation underscored a significant challenge for \tool: aligning with the authentic design intentions of software projects. We anticipate that offering a top-5 recommendation list could mitigate this challenge by presenting users with a spectrum of potential solutions. The discussion also underscores the importance of meaningful collaboration between tool developers and code maintainers. Such interactions are pivotal for advancing APR research, enhancing the practical impact, and facilitating its adoption in real-world software development scenarios.

==> sec/tool-bak.tex <==

\subsubsection{Dependency Graph Construction}
We define a Code Element Dependency Graph (CEDG) as an abstract representation of code elements relationships, which implies information on how a code element related to another. Formally, CEDG is regarded as a directed graph $G = (N_{ele}, DE)$, where:
\begin{itemize}[leftmargin=*]
    \item $N_{ele}$ represents code elements in the Rust program with key localization data including file paths, column and row numbers. $N_{ele}$ covers all the basic syntax elements that may appear in Rust. 
    \item $DE = \{(s_{1}, e_{1}), (s_{2}, e_{2}), ...\}$ is the set of Dependency Edges, where source element $s_{i}$ and related element $e_{i} \in N_{ele}$.
\end{itemize}

\yb{TODO: Figure about CEDG}

Building upon the High-Level Intermediate Representation (HIR), \tool firstly constructs a dependency graph that elucidates additional, potentially related, suspect locations. We drew upon the concept of \textit{abstract system dependence graph (ASDG)} as proposed by Chen\cite{chen2000graph} et al. In a similar manner to our CEDG, ASDG encodes components in the C language, including functions and global variables, to deal with feature location.

We conduct dependency analysis utilizing the High-level Intermediate Representation (HIR), which serves as one of the intermediary forms during Rust's compilation process. In order to build the Control and Data Flow Edge Graph (CEDG), we undertake a traversal of the let statements and assignment expressions within the HIR. This traversal relies on APIs provided by rustc. For let statements, the pattern and corresponding type are contingent on the initializer expression, implying that data flows from the initializer expression to the pattern. Similarly, in assignment expressions, the variables on the left-hand side (LValue) are dependent on the right-hand side (RValue). Specifically, when it comes to call and methodcall expressions, there may exist dependencies in the parameters in the call, so we delve deeper into the call to uncover additional dependencies. Leveraging the transitivity of the dependency relationship, we iteratively construct the CEDG.



\subsubsection{Fault Localization}
When a panic occurs in a Rust program, it initiates the unwinding process, where Rust meticulously traces back up the stack, ensuring the orderly cleanup of resources. Concurrently, an error message, rich with crucial details, is generated. This message is further supplemented with a backtrace if the RUST\_BACKTRACE environment variable is engaged, providing in-depth diagnostics. 
\tool harnesses this backtrace, deploying regular expressions to distill key localization data, including file paths, column, and row numbers. 

Building on the initial locations provided by the backtrace, we proceed to explore the CEDG for additional related suspicious locations. This process yields a compilation of locations, which, at this stage, remain in a disordered sequence. To rank these suspicious locations, we then refer to the structual similarity proposed by Laura~\cite{laura2014dep} et.al. Given that the exact buggy locations might not be directly revealed in the stack trace\cite{schroter2010stacktrace}, Laura posited that the true location of a bug is likely to share structural similarities with the functions outlined in the stack trace, a hypothesis that has been substantiated. Accordingly, we define structural similarity based on the minimum distance between a Rust code element \textit{e} and the locations within a backtrace triggered by a panic. This distance is mathematically represented as follows:

\begin{equation}\label{eq:dist}
\text{dist}(\text{backtrace}, e) = \text{shortestPath}(l, e), \quad \forall l \in \text{backtrace}
\end{equation}

Notice that when the code element \textit{e} is directly listed in the backtrace, the computed distance will be zero, indicating an exact match with the error location. Conversely, if there is no identifiable path connecting the code element \textit{e} to any location within the backtrace, the distance is defined as infinite, signaling a lack of direct correlation with the reported error.

Formula ~\ref{eq:simi_loc} defines the similarity score $simi_{\text{loc}}$ normalized by a constant 
$\lambda$, which ensures that the score is scaled within a meaningful range. 

\begin{equation}\label{eq:simi_loc}
    simi_{\text{loc}} = 1 - \frac{\min(\text{dist}(\text{backtrace}, e), \lambda)}{\lambda}, \quad \lambda \geq 1
\end{equation}

In a series of extensive and meticulous experiments, Lobster~\cite{laura2014dep} illustrates that setting $\lambda$ to 1, which corresponds to disregarding dependency entirely, results in the least effective similarity score. It is recommended that a value of $\lambda = 2$ be adopted for optimal performance. Following the recommendation, \tool is configured with $\lambda$ set to 2. This adjustment entails incorporating both the precise locations within the backtrace and the code elements that are in a dependent relationship with those identified in the backtrace, ensuring a more comprehensive analysis.

\tool adeptly calculates \textit{a suspicion score} for each location by applying the formula defined as follows:

\begin{equation}\label{eq:score_loc}
score_{\text{loc}} = N \times \left( \frac{1}{\text{D}} + simi_{\text{loc}} \right),
\end{equation}
in which $N$ denotes the frequency of occurrences of a specific file within the backtrace, and $D$ represents the depth of the location in the backtrace sequence.

This calculated metric forms the basis for generating a prioritized list of fault locations, aiding in the swift identification and resolution of errors. Formula ~\ref{eq:score_loc} incorporates the frequency of file appearances, premised on the notion that a higher occurrence rate of a file in the stack trace significantly elevates the likelihood of it harboring the suspect location. The rationale behind this approach is intuitive: files that recur frequently in diagnostics are often more integral to the execution path that led to the error, hence more likely to be relevant to the fault. Furthermore, Formula ~\ref{eq:score_loc} accounts for the stack's depth, where a shallower depth is indicative of a closer relationship to the origin of the error, thus increasing the file's suspicion score. 

It appears that despite numerous approaches claiming performance improvements, there has been little adoption of Automatic Program Repair research or practices. This lack of adoption could be attributed to issues with coarse-grained fault localization, as discussed by Koyuncu et al.~\cite{koyuncu2019ifixr}. It's crucial to emphasize that, in contrast, \tool employs fault localization at the expression level. This detail will be further elaborated in Section~\ref{subsec:rq1}. Such a granular approach to fault localization significantly enhances the applicability of our method in real-world scenarios.




\subsubsection{Pattern-based Patch Generation}



Based on the detected suspicious locations' list, \tool iteratively attempts to match each of these locations with the mined fix patterns, which are illustrated in Section~\ref{subsec:pattern_mining}. 
% Each pattern consists of an edit script applied to specific Abstract Syntax Tree (AST) nodes, which serve as the context for matching fix patterns. 
Specifically, \tool parses the suspicious file to AST, and perform transformations according to the localized expression with row and column number.
\liu{@yunbo: Are all the patterns executed here, or is only one selected for execution? If only one is selected, what is the basis?}

Considering that there may be multiple suspicious locations and matched patterns, resulting in multiple combination of fixes, we first validate the generated patches, and then further sort the generated patches based on the validation results and relevance assessment.



\smallskip
\textbf{Patch validation.} 
% The comprehensive process, encompassing both fault localization and patch generation, yields multiple patch candidates for each identified Rust panic bug. 
% The generation of high-quality patches plays a crucial role in the overall quality of repairs, highlighting the importance of not only identifying faults but also rectifying them effectively. 
% Moreover, addressing the issue of patch overfitting is essential to ensure the selection of genuinely effective patches, avoiding solutions that merely succeed in passing the current test suite without genuinely correcting the underlying bug.
For APR task, it is important to guarantee that the generated patches repair the panic bugs as well as do not affect the semantics of the original program.
In our work, we incorporate \textit{cargo-test}, a built-in tool in Rust's package manager, to automate the execution of regression tests within a package. 
After performing the validation, the patches would have several cases: 
(1) The panic bug is fixed and all the test cases in the crate execute with the same result as before.
Our goal is to generate these patches, which indicates the most likely correct fix.
(2) The panic bug is fixed but the execution results of some test cases are not consistent with the original program.
This suggests that the fix code may have introduced some logical modifications that cause the semantic inconsistency, and may need to be manually checked for further confirmation.
(3) The panic bug is not fixed and we don't evaluate the regression testing because it's not a correct fix.


% This approach mirrors the strategy adopted by \textit{iFixR}~\cite{koyuncu2019ifixr}, whereby our tool, \tool, does not anticipate future test scenarios for selecting patch candidates. This limitation is intentional to emulate the conditions of real-world fix applications, where future test cases are unknown at the time of repair. Instead, our reliance is placed on regression testing to guarantee that the chosen patches do not alter the original functionality of a Rust crate adversely. It is important to note that we employ the \textit{--all-features} option to ensure all available features of all targeted packages are activated during testing.
% This methodology ensures that \tool selects patches that not only address the immediate issue—manifested as a panic in the Rust program—but also maintain the integrity and expected behavior of the entire software package. 
The validation results are further applied to \tool to output the final patch ordering.
By focusing on regression testing, we can effectively filter out patches that might introduce new errors or exhibit overfitting to the test suite, thereby enhancing the reliability and robustness of the repair process.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\smallskip
\textbf{Patch prioritization.}

\liu{@yunbo: Add the details of patch ordering, the correlation, validation results, etc., all these things should be considered when ordering.}
\liu{It seems that the follow words are related, but you need to rewrite them into a technique version, rather than trivial introduction.}

The order of this list primarily depends on two factors, which are also two types of information provided when Rust panic is triggered:

\begin{enumerate}[leftmargin=*]
    \item Location: During the Fault Localization process, \tool generates a ranked list of suspicious locations, each accompanied by a suspicious score. This score indicates the likelihood of the corresponding location being the precise fix location. This information is crucial in determining the final recommended list, as it aids in prioritizing potential fixes based on their probability of addressing the issue effectively. 
    \item Error message: Typically, the panic! macro is accompanied by an error message that provides specific details about the reason for the panic bug. For instance, an error message might resemble 'attempt to subtract with overflow', originating from syn-3 in our \dataset. This message underscores the occurrence of an arithmetic overflow. Consequently, a patch utilizing an overflow-related fix pattern tends to rank higher in the final list. 
\end{enumerate}

By leveraging TF-IDF techniques to calculate the textual similarity between the detailed description and the panic error message, \tool combines this similarity with the suspicious score in Fault Location to produce the ultimate score of a patch. 
This combined score is used to rank the patches in descending order, ensuring that patches with higher scores are prioritized at the top of the recommendation list. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\smallskip
\textbf{Output.}
\tool finally outputs a ranked recommendation list of patches along with explanations in natural language, thus alleviating the problem of patch interpretability~\cite{}.
Specifically, we define a corresponding natural language description template for each fix pattern, where the variable names and localization information are populated based on the results extracted from the error localization performed by \tool.
This description offers comprehensive insights into the modifications made and the specific patterns utilized in the patch. 
Finally, \tool presents the top 5 patches with the highest scores, providing users with the most promising solutions for addressing the panic bug.




\smallskip
\textbf{A running example.}
\liu{@yunbo: This example is not OK, everyone knows that a pattern needs to be applied, the key here should be how that pattern is chosen. Change it to a more complex example, or even one with multiple rounds of fixes. The process of pattern matching needs to be represented, such as the original error code and panic backtrace messages, and then illustrate the step for pattern ordering. The AST is not needed.}

% \begin{listing}[h]
% \begin{minted}[linenos=true,
% firstnumber=180,
% fontsize=\small,
% xleftmargin=15pt,
% highlightcolor=red!10,
% highlightlines={189}]{rust}
% if let Some(span) = duration.num_nanoseconds() { // span
%     if naive.timestamp().abs() > 
%         MAX_SECONDS_TIMESTAMP_FOR_NANOS {
%         return Err(RoundingError::TimestampExceedsLimit);
%     }
%     let stamp = naive.timestamp_nanos(); // stamp
%     if span > stamp.abs() {
%         return Err(RoundingError::DurationExceedsTimestamp);
%     }
%     let delta_down = stamp % span; // panic!
% }
% \end{minted}
% \caption{A code snippet from Rust crate chrono.} \label{lst:ex_fl}
% \end{listing}

% Listing ~\ref{lst:ex_fl} showcases an actual code snippet sourced from our dataset, which originates from the Rust crate chrono. In this segment, the declaration of the variable \textit{delta\_down} precipitates a panic as the value of span may be zero. This variable is initialized with a binary expression that integrates two other variables, \textit{stamp} and \textit{span}. Through the analysis conducted via the Code Element Dependency Graph (CEDG), a dependency linkage between \textit{delta\_down} and these two variables is established. Consequently, this generates the following dependency representation: The variable \textit{delta\_down} is found to depend on \textit{stamp} and \textit{span} due to its initialization from a binary operation involving both. In the context of the CEDG, \textit{delta\_down} is directly connected to \textit{stamp} and \textit{span}, illustrating their integral roles in its computation. This discovered dependency allows \tool to further explore the definition of \textit{span} for potential corrections. This association is critical for understanding the panic's causality, as it reveals the flow of data leading to the fault. 


% \begin{listing}[h]
% \begin{minted}[linenos=false,
% fontsize=\small,
% xleftmargin=10pt,
% highlightcolor=red!10,
% highlightlines={2}]{rust}
% pub fn pop_if_empty(&mut self) -> &mut Self {
%     if self.url.serialization[self.after_first_slash..]
%         .ends_with('/') 
%     {
%         self.url.serialization.pop();
%     }
%     self
% }
% \end{minted}
% \caption{A code snippet from Rust crate percent-encoding.} \label{lst:ex_patch}
% \end{listing}



Consider the example of a panic triggered by the Rust crate percent-encoding, as provided in Listing ~\ref{lst:fix}. This panic occurs when the start of the range expression in the index expression \\ \textit{self.url.serialization} may exceed its boundary. \tool initially parses the path-segments.rs file into an AST, which includes the if expression depicted in Figure ~\ref{fig:ast}. Subsequently, \tool matches a fix pattern associated with the if expression, introducing an additional condition to prevent the out-of-index panic. This method can be matched against two types of context: the name of the array and the index in the range expression. 

Upon retrieving all the necessary information, \tool assigns the fix pattern, modifying the if condition to include a length check between the start of the range expression and the length of the index expression. Furthermore, \tool will match other fix patterns for the sub-expressions in the if expression in Listing \ref{lst:fix}, such as the index expression, respectively and successively.

\begin{listing}
\begin{minted}[linenos=false,
fontsize=\small]{diff}
-  if self.url.serialization[self.after_first_slash..]
-      .ends_with('/') 
+  if self.after_first_slash < self.url.serialization.len()
+      && self.url.serialization[self.after_first_slash..]
+      .ends_with('/')
\end{minted}
\caption{A fix pattern is applied to the panic from Rust crate percent-encoding.} \label{lst:fix}
\end{listing}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/fig_ast.png}
    \textit{\small{*"raw\_code" denotes the source code at the node position.}}
    \caption{AST of panic from Rust crate percent-encoding.}
    \label{fig:ast}
\end{figure}

%%%%%%%%%%%%%%%%% example %%%%%%%%%%%%%%%%%%%
